Deterministic Algorithms for Decremental Shortest Paths via Layered Core Decomposition

In the decremental single-source shortest paths (SSSP) problem, the input is an undirected graph $G=(V,E)$ with $n$ vertices and $m$ edges undergoing edge deletions, together with a fixed source vertex $s\in V$. The goal is to maintain a data structure that supports shortest-path queries: given a vertex $v\in V$, quickly return an (approximate) shortest path from $s$ to $v$. The decremental all-pairs shortest paths (APSP) problem is defined similarly, but now the shortest-path queries are allowed between any pair of vertices of $V$. Both problems have been studied extensively since the 80's, and algorithms with near-optimal total update time and query time have been discovered for them. Unfortunately, all these algorithms are randomized and, more importantly, they need to assume an oblivious adversary. Our first result is a deterministic algorithm for the decremental SSSP problem on weighted graphs with $O(n^{2+o(1)})$ total update time, that supports $(1+\epsilon)$-approximate shortest-path queries, with query time $O(|P|\cdot n^{o(1)})$, where $P$ is the returned path. This is the first $(1+\epsilon)$-approximation algorithm against an adaptive adversary that supports shortest-path queries in time below $O(n)$, that breaks the $O(mn)$ total update time bound of the classical algorithm of Even and Shiloah from 1981. Our second result is a deterministic algorithm for the decremental APSP problem on unweighted graphs that achieves total update time $O(n^{2.5+\delta})$, for any constant $\delta>0$, supports approximate distance queries in $O(\log\log n)$ time; the algorithm achieves an $O(1)$-multiplicative and $n^{o(1)}$-additive approximation on the path length. All previous algorithms for APSP either assume an oblivious adversary or have an $\Omega(n^{3})$ total update time when $m=\Omega(n^{2})$.

==> APSP-large-distance.tex <==

\subsection{Large-Distance Regime}\label{subsection: APSP: large distance}
In this subsection we provide the proof of Theorem~\ref{thm: main for APSP w distance bound}, assuming that $D\geq \sqrt{n}$. As stated before, our algorithm will provide slightly stronger guarantees: if $D\leq \dist(u,v)\leq 2D$, the algorithm will return a path connecting $u$ to $v$ of length at most  $(1+\eps)\dist(u,v)$. The total expected update time of the algorithm becomes $\tilde O\left (n^{2.5}\log (1/\eps)/\eps^2\right )$, and the expected time to respond to a query is $O(n\poly\log n\log(1/\eps))$.
The algorithm combines our algorithm for \SSSP with moving \ESTs of Henzinger et al.~\cite{henzinger16}.

We start by setting the virtual degree threshold $\highlightf{\tau=\frac{8n \alpha}{\eps D}}$, where $\alpha=O(\poly\log n)$ is such that the algorithm from Theorem \ref{thm: responding to short-paths queries in heavy graph} is guaranteed to return, in response to each query $\shortpath(C,u,v)$, a path of length at most  $|V(C)|\alpha /\tau$ connecting $u$ to $v$. We define the heavy graph $G^H=H_{\tau}(G)$ -- the subgraph of $G$ induced by all vertices whose virtual degrees are at least $\tau$.
In other words, if we let $U=\set{v\in V(G)\mid \td(v)\geq \tau}$, then $G^H=G[\tau]$.

We also maintain the light graph $G^L\subseteq G$, defined as follows: $V(G^L)=V(G)$. For every vertex $v\in V(G)$ with $\td(v)<\tau$, we add all edges that are incident to $v$ in $G$ to graph $G^L$. Recall that, from Corollary~\ref{cor: few edges incident to Lambdaj}, the total number of edges of $G$ that ever belong to $G^L$ over the course of the algorithm is bounded by $O(n\tau)=\tilde O(n^2/(\eps D))$. 

Finally, we define the extended light graph $\hat G^L$, exactly as before. We start with $\hat G^L=G^L$; the vertices of $G^L$ are called \emph{regular vertices}. Next, for every connected component $C$ of $G^H$, we add a vertex $v_C$ to $\hat G^L$, that we call a \emph{special vertex}, and connect it to every vertex $u\in C$ with an edge of length $1/4$. %

We use two distance thresholds: the \emph{covering radius} $R^c=\eps D/4$, and the \emph{range radius} $R^d=2D$.

Throughout the algorithm, we will maintain a collection of \emph{centers}, located at verticecs of $\hat G^L$. For each such center, we will maintain an \EST whose source is the center. During the execution of the algorithm, we will sometimes open new centers, and construct a new \EST from that center. We may also \emph{move} some centers. Because of this, following~\cite{henzinger16}, we distinguish between the centers themselves and their locations. Therefore, we maintain a set $S=\set{s_1,s_2,\ldots,s_z}$ of centers, and for each $1\leq i\leq z$, we let $u_i\in V(\hat G^L)$ be the \emph{location} of the center. For each $1\leq i\leq z$, we maintain an \EST $T_i=\EST(\hat G^L,u_i,R^d)$, whose source is $u_i$, up to distance $R^d$. Note that, in addition to standard edge deletions, graph $\hat G^L$ also undergoes edge insertions (when the virtual degree of some vertex $x$ falls below $\tau$, we need to insert all edges incident to $x$ to $\hat G^L$), and also ``splitting'' of super-nodes (when some connected component $C$ of $G^H$ breaks into connected components $C_1$ and $C_2$, we need to update $\hat G^L$ accordingly, by replacing the supernode $v(C)$ with two new supernodes, $v(C_1)$ and $v(C_2)$. Therefore, we cannot apply the \EST algorithm as a black box. However, all these issues were dealt with in previous work~\cite{BernsteinChechik,fast-vertex-sparsest}. 

In order to analyze the running time of the \EST algorithm, and in order to simplify the analysis of the moving-center data structure, it is convenient to work with vertex potentials, that we define next.

Consider some center $s_i\in S$. For every vertex $u\in V(\hat G^L)$, we define the \emph{potential $\phi_{s_i}(u)$ of $u$ with respect to $s_i$}, as follows.

First, we define $\delta_{u_i}(u)=\max\set{0,R^d-\dist(u,u_i)}$. Intuitively, if $u\in V(T_i)$, then $\delta_{u_i}(u)$ is the amount by which $\dist(u,u_i)$ may grow until $u$ is deleted from the tree $T_i$. We are now ready to define the potential $\phi_{s_i}(u)$. We let $\alpha'=\hat c \log n$ for some large enough constant $\hat c$.


\begin{itemize}
	\item If $u$ is a regular vertex with $\td(u)<\tau$, then we let $\phi_{s_i}(u)=\alpha'\delta_{u_i}(u)\cdot \deg_G(u)$.
	\item If $u$ is a regular vertex with $\td(u)\geq \tau$, then we let $\phi_{s_i}(u)=4\alpha'\delta_{u_i}(u)\cdot \tau$.
	\item Finally, if $u=v(C)$ is a super-node, then we let $\phi_{s_i}(u)=4\alpha'\delta_{u_i}(u)|C|\log |C|$.
\end{itemize}

We let $\phi_{s_i}=\sum_{u\in V(\hat G^L)}\phi_{s_i}(u)$. For every vertex $u\in V(\hat G^L)$, we also define $\phi(u)=\sum_{s_i\in S}\phi_{s_i}(u)$, and we let $\phi=\sum_{u\in V(\hat G^L)}\phi(u)$. 

We will use the following theorem in order to maintain \ESTs from the centers $s_i$. The proof uses standard techniques and is deferred to the appendix.

\begin{theorem}\label{thm: maintain a single ES tree}
	There is an efficient algorithm, that, given a location $u_i$ of a center $s_i$, maintains \EST $T_i=\EST(\hat G^L,u_i,R^d)$. Moreover, if we denote by $\phi^0_{s_i}$ the potential $\phi_{s_i}$ when the tree was first constructed, by $\phi^t_{s_i}$ the potential $\phi_{s_i}$ after $t$ udates, and by $\eta^t$ the total time spent by the algorithm on processing the first $t$ updates, then $\phi^t_{s_i}+\eta^t\leq \phi^0_{s_i}$. The data structure takes time $O(|E(\hat G^L))$ to initialize.
\end{theorem}

We note that the updates that the algorithm from Theorem~\ref{thm: maintain a single ES tree} handles are (i) deletions of edges from $\hat G^L$; (ii) insertion of edges incident to vertices whose virtual degree has fallen below $\tau$; and (iii) splitting of supernodes $v(C)$.


In addition to the trees $\set{T_i}_{s_i\in S}$, we maintain the data structure \LCD from Theorem~\ref{thm: responding to short-paths queries in heavy graph} for the heavy graph $G^H$. Recall that the total expected update time of the data structure is $\tilde O(n^2)$, and the data structure supports queries  $\shortpath(C,u,v)$: given a connected component $C$ of $G^H$, return a path connecting $u$ to $v$ of length at most $\alpha |V(C)|/\tau)$. The running time for responding to a query is $O(|V(C)|\poly\log n)$. The algorithm may return ``Fail'' at any time; the probability of that happening over the whole run of the algorithm is at most $1/\poly(n)$.

We say that a vertex $u\in V(\hat G^L)$ is \emph{covered} by a center $s_i$ iff $\dist(u_i,u)\leq R^c$. Throughout the algorithm, we maintain 
the following invariant:

\begin{properties}{I}
	\item Throughout the algorithm, every vertex of $\hat G^L$ is covered by some center in $S$.\label{Invariant: every vertex is covered}
\end{properties}

We now proceed as follows. We first provide an algorithm for responding to shortest-path query. The algorithm is very similar to that employed in Section \ref{sec: SSSP}



-------------------------------------




Fix an index $1\leq i\leq \lambda$, and let $G_i$ be the sub-graph of $G$ induced by the edges in $E^i$, and let $G_i^H=H_{\tau_i}(G_i)$ be the corresponding heavy graph; reacall that $G_i^H$ is the sub-graph of $G_i$ induced by vertices whose virtual degrees are below $\tau_i$. For each $1\leq i\leq \lambda$, we maintain the \LCD data structure in $G_i^H$ in order to support queries $\shortpath(C,u,v)$ from Theorem~\ref{thm: responding to short-paths queries in heavy graph}. Recall that the total expected update time for each such data structure is $\tilde O(n^2)$, and so the total expected update time of all these data structures is $\tilde O(n^2\log L)$.
Whenever any of the algorithms from Theorem~\ref{thm: responding to short-paths queries in heavy graph} returns ``Fail'' (which happens with probability at most $1/\poly(n)$, we restart the whole algorithm from scratch. Note that the expected running time remains $\tilde O(n^2\log L)$.


==> APSP.tex <==

\section{APSP}\label{sec: APSP}
The goal of this section is to prove Theorems~\ref{thm: main for APSP} and~\ref{thm: main for APSP long range}. 
We consider each distance scale separately. 
We provide two different algorithms, one that works better when the target distance $D$ is large, and another that works better for small distances.

\begin{theorem}\label{thm: main for APSP w distance bound: large dist}
        There is a randomized algorithm, that, given parameters $0<\eps<1/2$ and $D>0$, and a simple undirected $n$-vertex graph $G$ with unit edge lengths that undergoes edge deletions, supports queries $\pquery_D(u,v)$ and $\distquery_D(u,v)$ for pairs of vertices $u,v$ that lie in the same connected component of $G$. Given a query $\pquery_D(u,v)$, the algorithm either correctly establishes that $\dist_G(u,v)>2D$, or it correctly establishes that both $u$ and $v$ lie in a connected component of $G$ containing fewer than $D$ vertices (so $\dist_G(u,v)<D$ must hold), or it returns a path connecting $u$ to $v$, of length at most $8D$. Moreover, if $D\leq \dist(u,v)\leq 2D$, then it is guaranteed to return a path  from $u$ to $v$ of length at most $(1+\eps)\dist(u,v)$. For each query $\distquery_D(u,v)$, the algorithm either correctly establishes that $\dist_G(u,v)<D$, or that $\dist_G(u,v)>(1+\eps)D$, or it returns an estimate $\dist'(u,v)$ such that $\dist_G(u,v)\leq \dist'(u,v)\leq (1+\eps)\dist_G(u,v)$, and $D\leq \dist'(u,v)\leq (1+\eps)^2D$.
        The algorithm works against an adaptive adversary. The total expected update time of the algorithm is $O\left (n^{3}\pln/(\eps^2 D)\right )$; each $\distquery_D$ is answered in $O(1)$ time, and each $\pathquery_D$ is answered in expected time $\tilde O(n)$.
\end{theorem}




\begin{theorem}\label{thm: main for APSP w distance bound: small dist}
        There is a randomized algorithm, that, given parameters $k\geq 1$ and $D>0$, and a simple undirected $n$-vertex graph $G$ with unit edge lengths that undergoes edge deletions, supports queries $\pquery_D(u,v)$ and $\distquery_D(u,v)$  for pairs of vertices $u,v$ that lie in the same connected component of $G$. Given query $\pquery_D(u,v)$, the algorithm returns a path from $u$ to $v$ in $G$, of length is at most $2^{k+1}D+\log^{O(k)}n$, if $D\leq \dist(u,v)\leq 2D$; otherwise, it either returns an arbitrary path connecting $u$ to $v$, or it returns an empty path. Given query $\distquery_D(u,v)$, such that $u$ and $v$ lie in the same connected component of $G$, the algorithm returns either ``Yes'' or ''No''; if the algorithm returns ``Yes'', then we are guaranteed that $\dist_G(u,v)\leq 2^{k+1}D+\log^{O(k)}n$, and if it returns ``No'', then we are guaranteed that $\dist_G(u,v)>2D$. The algorithm works against an adaptive adversary. The total expected update time  is  $O(n^{2.5+3/(2k)}\cdot \sqrt{D} )\cdot \log^{O(k)}n$; each query $\distquery_D(u,v)$ is answered in time $O(1)$, and each query $\pathquery_D(u,v)$ is answered in expected time $\tilde O(n^{1+1/k})$.
\end{theorem}


We now complete the proof of Theorem~\ref{thm: main for APSP} using Theorems~\ref{thm: main for APSP w distance bound: large dist} and~\ref{thm: main for APSP w distance bound: small dist}. We fix $\eps$ to be some constant between $0$ and $1/2$. For all $1\leq i\leq \log_{1+\eps}n$, let $D_i=(1+\eps)^i$. Let $D^*=n^{1/3-3/(4k)}$. For all $D_i\leq D^*$, we maintain the data structure from Theorem~\ref{thm: main for APSP w distance bound: small dist} with the bound $D_i$, and for all $D_i>D^*$, we maintain the data structure from Theorem~\ref{thm: main for APSP w distance bound: large dist}. A simple accounting shows that the total expected update time needed to maintain these data structures is bounded by $O(n^{8/3+3/(4k)}\cdot \log^{O(k)}n)$. Additionally, we need an algorithm that efficiently responds to connectivity queries. We use the results of~\cite{conn-fast-query}, who provide a deterministic data structure, that, given a dynamic graph $G$, responds to connectivity queries within $G$ in $O(1)$ time per query, and has amortized update time $\tilde O(n^{1/3})$ per operation. Since we only need to handle edge deletions, the total update time of this data structure is $\tilde O(mn^{1/3})=\tilde O(n^{7/3})$.














We now show how path and distance queries are handled. Given a query $\pathquery(x,y)$, we first check whether $x$ and $y$ lie in the same connected component of $G$, in time $O(1)$. If this is not the case, then we terminate the algorithm and report this. Otherwise, we simply run queries $\pathquery_{D_i}(x,y)$ for all values $D_i$, where we use the algorithm from Theorem~\ref{thm: main for APSP w distance bound: small dist} for values $D_i\leq D^*$ and the algorithm from Theorem~\ref{thm: main for APSP w distance bound: large dist} for $D_i>D^*$. We then return the shortest $x$-$y$ path that any of these queries has returned. We are guaranteed that the length of the path is at most $2^{k+1}\dist_G(x,y)+\log^{O(k)}n$. If no path is ever returned, then we are guaranteed that $x$ and $y$ are not connected in $G$. The total expected running time to respond to $\pathquery(x,y)$ is at most $\tilde O(n^{1+1/k})$. 

Finally, assume that we are given a query $\distquery(x,y)$. We start by checking, in $O(1)$ time, whether $x$ and $y$ lie in the same connected component of $G$. If this is not the case, we terminate the algorithm and report this. Otherwise, we perform a binary search on the values $D_i$. Given such a value $D_i$, we run $\distquery_{D_i}(x,y)$ using the algorithm from Theorem~\ref{thm: main for APSP w distance bound: large dist} or~\ref{thm: main for APSP w distance bound: small dist}, depending on the value of $D_i$. In either case, we will either correctly establish that $\dist_G(x,y)\leq 2^{k+1}D_i+\log^{O(k)}n$, or that $\dist_G(x,y)>(1+\eps)D_i$, which will allow us to narrow down the scope of the binary search. Since each query $\distquery_D(x,y)$ is processed in time $O(1)$, and since there are $O(\log n)$ possible values of $D_i$, the total time to respond to $\distquery(x,y)$ is $O(\log\log n)$.


Lastly, to complete the proof of Theorem~\ref{thm: main for APSP long range}, we set $D^*=n^{\delta}$, and we only use values $D_i\geq D^*$, with Theorem~\ref{thm: main for APSP w distance bound: large dist}. This guarantees that the total expected update time of the algorithm is $\tilde O(n^{3-\delta}/\eps^2)$.
We respond to queries $\distquery(x,y)$ using the same algorithm as before, except that we ignore values $D_i<D^*$. Therefore, the algorithm either correctly establishes that $\dist_G(x,y)<n^{\delta}$, or returns a $(1+\eps)$-approximation to $\dist_G(x,y)$. In the former case, we return the value $n^{\delta}$ in response to the query, and in the latter case we return the approximate estimate.
The query time for $\distquery$ remains $O(\log\log n)$.

In order to support $\pathquery$, we additionally maintain the connectivity/spanning forest data structure $\CONNSF(G)$. Given a query $\pathquery(x,y)$, we first run $\distquery(x,y)$ to obtain an approximate estimate $\dist'(x,y)$ on $\dist(x,y)$. If this estimate is at least $n^{\delta}$, then we use $\distquery_{D_i}(x,y)$ with the appropriate value $D_i$ to obtain a $(1+\eps)$-approximate shortest $x$-$y$ path. 
If the estimate is below $n^{\delta}$, then we use $\distquery_D(x,y)$ with $D=n^{\delta}$. If the outcome is a path connecting $x$ to $y$, whose length is at most $4D$, then we return this path. Otherwise, we are guaranteed that $x$ and $y$ lie in the same connected component $C$ of $G$, that contains fewer than $D$ vertices. We can then use the Steiner Forest from $\CONNSF(G)$ data structure in order to obtain a path of length at most $D$ connecting $x$ to $y$ in $C$, in total time $O(D)=O(n^{\delta})$. The total expected query time for $\distquery$ is $\tilde O(n)$.


The remaining of this section is organized as follows.
In \Cref{subsection: APSP: large distance}, we prove \Cref{thm: main for APSP w distance bound: large dist} by giving a data structure for the large distance regime. \Cref{APSP: small dist,APSP: small-distance dense,subsec: DS for light graph} are for proving \Cref{thm: main for APSP w distance bound: small dist}. Roughly, \Cref{APSP: small-distance dense} describes the data structure for the dense parts, and \Cref{subsec: DS for light graph} is for the sparse parts.

\subsection{The Large-Distance Regime}\label{subsection: APSP: large distance}
In this subsection we provide the proof of Theorem~\ref{thm: main for APSP w distance bound: large dist}. %
The algorithm combines our algorithm for \SSSP with the moving  \EST data structure of Forster et al.~\cite{henzinger16}. As in the proof of Theorem \ref{thm: responding to short-paths queries in heavy graph}, we set $\Delta=2$, and we define the virtual vertex degrees in $G$ with respect to this value of $\Delta$.

We start by setting the virtual degree threshold ${\tau=\frac{8n \alpha}{\eps D}}$, where $\alpha=O(\poly\log n)$ is such that the algorithm from Theorem \ref{thm: responding to short-paths queries in heavy graph} is guaranteed to return, in response to each query $\shortpath(C,u,v)$, a path of length at most  $|V(C)|\alpha /\tau$ connecting $u$ to $v$. Notice that we can ensure w.l.o.g. that $\tau$ is large enough (e.g., $\tau>1000$) by increasing the value of $\alpha$ as needed. We define the heavy graph $G^H=H^{\tau}(G)$ -- the subgraph of $G$ induced by all vertices whose virtual degrees are at least $\tau$.
In other words, if we let $U=\set{v\in V(G)\mid \td_G(v)\geq \tau}$, then $G^H=G[U]$.

We also maintain the light graph $G^L\subseteq G$, defined as follows: $V(G^L)=V(G)$; for every vertex $v\in V(G)$ with $\td_G(v)<\tau$, we add all edges that are incident to $v$ in $G$ to graph $G^L$. Recall that, from Corollary~\ref{cor: few edges incident to Lambdaj}, the total number of edges of $G$ that ever belong to $G^L$ over the course of the algorithm is bounded by $O(n\tau)=\tilde O(n^2/(\eps D))$. 

Finally, we define the extended light graph $\hat G^L$, as follows. We start with $\hat G^L=G^L$; the vertices of $G^L$ are called \emph{regular vertices}. Next, for every connected component $C$ of $G^H$, we add a vertex $v_C$ to $\hat G^L$, that we call a \emph{special vertex}, or a \emph{supernode}, and connect it to every vertex $u\in V(C)$ with an edge of length $1/4$. %
The following 
is immediate from the assumption that all edge lengths in $G$ are at least $1$.

\begin{observation}\label{obs: distances in G and light graph for APSP}
        Throughout the algorithm, for every pair of vertices $x,y\in V(G)$, $\dist_{\hat G^L}(x,y)\leq \dist_G(x,y)$.
\end{observation}

We use two distance thresholds: the \emph{covering radius} $R^c=\eps D/4$, and the \emph{range radius} $R^d=4D$.

Throughout the algorithm, we will maintain a collection of \emph{centers}, located at vertices of $\hat G^L$. For each such center, we will maintain an \EST whose source is the center, up to distance $R^d$. During the execution of the algorithm, we will sometimes open new centers, and construct new \ESTs from those centers. As in~\cite{henzinger16}, we may also \emph{move} some centers, from one location to another. Because of this, following~\cite{henzinger16}, we distinguish between the centers themselves and their locations. Therefore, we maintain a set $S=\set{s_1,s_2,\ldots,s_z}$ of centers, and for each $1\leq i\leq z$, we let $u_i\in V(\hat G^L)$ be the \emph{location} of the center. For each $1\leq i\leq z$, we maintain an \EST $T_i=\EST(\hat G^L,u_i,R^d)$, whose source is $u_i$, up to distance $R^d$. Note that, in addition to standard edge deletions, graph $\hat G^L$ also undergoes edge insertions (when the virtual degree of some vertex $x$ falls below $\tau$, we need to insert all edges incident to $x$ to $\hat G^L$), and also ``splitting'' of supernodes (when some connected component $C$ of $G^H$ breaks into connected components $C_1$ and $C_2$, we need to update $\hat G^L$ accordingly, by replacing the supernode $v_C$ with two new supernodes, $v_{C_1}$ and $v_{C_2}$). Therefore, we cannot apply the \EST algorithm as a black box. However, all these issues were dealt with in previous work~\cite{BernsteinChechik,fast-vertex-sparsest}, and we deal with them similarly.


\begin{definition}
For all $s_i\in S$ and $u\in V(\hat G^L)$, if $\dist_{\hgl}(u_i,u)\leq R^c$, then we say that center $s_i$ \emph{covers} $u$.
\end{definition}


In order to analyze the running time of the \EST algorithm, and in order to simplify the analysis of the moving-center data structure, it is convenient to work with vertex potentials, that we define next.


\paragraph{Vertex Potentials.}
Consider some center $s_i\in S$. For every vertex $u\in V(\hat G^L)$, we define the \emph{potential $\psi_{s_i}(u)$ of $u$ with respect to $s_i$}, as follows.

First, we define $\delta_{s_i}(u)=\max\set{0,R^d-\dist_{\hgl}(u,u_i)+1}$. Intuitively, if $u\in V(T_i)$, then $\delta_{s_i}(u)$ is the amount by which $\dist_{\hgl}(u,u_i)$ may grow until $u$ is deleted from the tree $T_i$. We are now ready to define the potential $\psi_{s_i}(u)$. We let $\hat c$ be a large enough constant.


\begin{itemize}
        \item If $u$ is a regular vertex with $\td_G(u)<\tau$, then we let $\psi_{s_i}(u)=\hat c\delta_{s_i}(u)\cdot \deg_{\hat G^L}(u)$.
        \item If $u$ is a regular vertex with $\td_G(u)\geq \tau$, then we let $\psi_{s_i}(u)=\hat c\delta_{s_i}(u)\cdot (8\tau+\deg_{\hat G^L}(u))$.
        \item Finally, if $u=v_C$ is a supernode, then we let $\psi_{s_i}(u)=128\hat c \delta_{s_i}(v_C)\cdot |C|\log^2 |C|$.
\end{itemize}

We let $\Psi_{s_i}=\sum_{u\in V(\hat G^L)}\psi_{s_i}(u)$. 
Note that, when a tree $T_i$ is constructed, potential $\Psi_{s_i}$ is bounded by $R^d\cdot (O(|E(\hgl)|+O(\tau n)+O(n\log^2n))=O(\tau n D\log^2n)=O(n^2\poly\log n/\eps)$, since $\tau=8n\alpha/(\eps D)$, and $\alpha=\poly\log n$. Once we construct the tree $T_i$, the potential $\Psi_i$ may only decrease (as we show later), except when we move the center $s_i$ to a new location. The increase will depend on the distance between the old and the new locations of $s_i$. Our algorithm will ensure that the total distance traveled by all centers is relatively small, and that the total number of centers we open is at most $O(n/(\eps D))$.
We let $\Psi=\sum_{s_i\in S}\Psi_{s_i}$ be the total potential. 



\subsubsection{Maintaining a Single \EST}
Recall that for every center $s_i\in S$, we maintain an $\EST$ $T_i=\EST(\hat G^L,u_i,R^d)$ from source $u_i$, up to distance $R^d$. We need the corresponding data structure to support the following update operations:

\paragraph{$\deledge(T_i,e)$:} given an edge $e=(x,y)$ with $x,y\in V(T_i)$, that is being deleted from $\hat G^L$, update the data structure of $T_i$ accordingly. 


\paragraph{$\splitsupernode(T_i,v_C,C_1,C_2):$} The input is a supernode $v_C\in V(T_i)$ corresponding to some connected component $C$ of $G^H$, together with names $C_1,C_2$ of the new connected components into which $C$ is split, such that $|C_1|\leq |C_2|$, and a list of vertices of $C_1$. We need to replace $v_C$ with $v_{C_1}$ and $v_{C_2}$, connecting every vertex of $C_1$ to $v_{C_1}$ and every vertex of $C_2$ to $v_{C_2}$ with edges of length $1/4$, and to update the data structure of $T_i$ accordingly.

\paragraph{$\insertedges(T_i,x,E'):$} the input is a vertex $x\in V(T_i)$ whose virtual degree  $\td_G(x)$ was at least $\tau$ and has just decreased to below $\tau$, and a set $E'$ of at most $\tau$ edges incident to $x$, that are inserted into $\hat G^L$. We will guarantee that the insertion of these edges does not decrease the distances between any pair of vertices of $\hat G^L$. The goal is to update the data structure of $T_i$ to reflect these edge insertions. 




We use the following theorem in order to maintain \ESTs from the  locations $u_i$ of centers $s_i$. The proof uses standard techniques and is deferred to Appendix.

\begin{theorem}\label{thm: maintain a single ES tree}
        There is a deterministic algorithm, that, given a location $u_i$ of a center $s_i\in S$, maintains \EST $T_i=\EST(\hat G^L,u_i,R^d)$, under $\deledge$, $\splitsupernode$, and $\insertedges$ update operations. Additionally, for every vertex $u\in V(\hat G^L)$ that belongs to $T_i$, it maintains a pointer from $u$ to its copy in $T_i$, and, if $u$ is covered by $s_i$, it maintains a pointer from $u$ to $u_i$. Moreover, if we denote by $\Psi^0_{s_i}$ the potential $\Psi_{s_i}$ right after the tree was first constructed, by $\Psi^t_{s_i}$ the potential $\Psi_{s_i}$ after $t$ updates, by $\eta^t$ the total time spent by the algorithm on processing the first $t$ updates, and by $m^t$ the total number of times the $\deledge$ operation was executed, then $\eta^t\leq \Psi^0_{s_i}-\Psi_{s_i}^t+O(m^t)$. The data structure takes time $O(|E(\hat G^L)|)$ to initialize; the initialization time is not included in the update time $\eta^t$.
\end{theorem}





\subsubsection{Maintaining the Data Structures}

In addition to the trees $\set{T_i}_{s_i\in S}$, we maintain the data structure \LCD from Theorem~\ref{thm: responding to short-paths queries in heavy graph} for the heavy graph $G^H$. Recall that Theorem~\ref{thm: responding to short-paths queries in heavy graph} uses the \LCD data structure with parameter $\Delta=2$; its total expected update time is $\tilde O(n^2)$; and the data structure supports queries  $\shortpath(C,u,v)$: given a connected component $C$ of $G^H$, return a path connecting $u$ to $v$ of length at most $\alpha |V(C)|/\tau$. The expected time for responding to a query is $O(|V(C)|\poly\log n)$. The algorithm may return ``Fail'' at any time; the probability of that ever happening over the whole run of the algorithm is at most $1/\poly(n)$.
If the algorithm ever returns ``Fail'', we simply recompute all data structures from scratch. Since the probability of this event is very low, it will not affect the asymptotic running time of our algorithm. Therefore, for convenience, from now on, we assume that the algorithm from Theorem~\ref{thm: responding to short-paths queries in heavy graph} never returns ``Fail''.

Additionally, we maintain a connectivity/spanning forest data structure $\CONNSF(G^H)$ for the heavy graph $G^H$.
For every vertex $u\in V(\hat G^L)$ of the light graph, and every center $s_i\in S$ with $u\in V(T_i)$, we also maintain a pointer from $u$ to its copy in $T_i$, and, if $s_i$ covers $u$, we maintain a pointer from $u$ to $u_i$; this is done using the data structure from Theorem~\ref{thm: maintain a single ES tree}.


We now describe an update operation when an edge $e=(x,y)$ needs to be deleted from the graph $G$. If $e\in E(G^L)$, then we delete $e$ from $G^L$. Additionally, for every tree $T_i$ with $s_i\in S$, such that both $x,y\in V(T_i)$, we run procedure $\deledge(T_i,e)$.

Assume now that $e\in E(G^H)$. We update the data structure from Theorem~\ref{thm: responding to short-paths queries in heavy graph} with the deletion of the edge $e$. As the result, we obtain a collection $X$ of vertices, whose virtual degrees were at least $\tau$ before edge $e$ was deleted, and fell below $\tau$ after. We let $E'$ be the set of all edges that are incident to the vertices of $X$ but do not belong to $\hat G^L$. Every edge in $E'$ is deleted from $G^H$ and needs to be inserted into $\hat G^L$. Additionally, as edges of $E'\cup \set{e}$ are deleted from $G^H$, some connected components of $G^H$ may decompose into smaller connected components, and we need to updte $\hat G^L$ accordingly. We now proceed in two steps. In the first step, we insert the edges of $E'$ into $\hat G^L$ and the \ESTs $T_i$ that we maintain, and in the second step, we handle the splitting of supernodes.


 Consider running procedure $\DP(G,\tau)$. Using the same arguments as before, we can run this procedure so that the vertices of $X$ are deleted from $J_1$ last, after all vertices that did not belong to $G^H$ at the beginning of the current update were deleted. Moreover, if $X=\set{x_1,\ldots,x_q}$, where the vertices are indexed in the order of their deletion from $J_1$, then for each $1\leq a\leq k$, there are at most $\tau$ edges connecting $x_a$ to $(x_{a+1},\ldots,x_q)\cup (V(H)\setminus X)$; we denote this set of edges by $E_a$. In other words, $E'=\bigcup_{a=1}^qE_a$, and for all $1\leq a\leq q$, $|E_a|\leq \tau$. 
 Notice that, if $e'=(x_a,y)$ is an edge of $E'$, then, before the deletion of $e$, edge $e'$ belonged to $G^H$, and in particular $x_a$ and $y$ belonged to the same connected component of $G^H$, that we denote by $C$. Therefore, vertex $v_C$ is currently present in graph $\hgl$, as well as edges $(x_a,v_C)$, $(y,v_C)$ of length $1/4$ each. It is then easy to see that the insertion of $e'$ into \hgl does not decrease distances between any pair of vertices. We consider the vertices $x_1,\ldots,x_q$ one-by-one. For each such vertex $x_a$, for every tree $T_i$ that contains $x_a$, we run the procedure $\insertedges(T_i,x_a,E_a)$. 
 Note that we do not need to run procedure $\DP(G,\tau)$ from scratch every time an edge of $G$ is deleted. Instead, we can maintain the partition $(J_1,J_2)$ from the previous time, so that we only need to move the vertices of $X$ from $J_1$ to $J_2$. If the algorithm that maintains the \LCD data structure also maintains the degrees of all vertices in $G$, then the additional running time needed to update the partition $(J_1,J_2)$ is bounded by $O(|E'|)$.
 The total running time spent on inserting all these edges into all the trees is asymptotically bounded by the update times of the $\insertedges(T_i,x_a,E_a)$ operations executed in this step, and we charge it to these operations.
 
 Lastly, we process every edge of $E'\cup \set{e}$ one-by-one. For each such edge $e'=(x,y)$, we update the connectivity data structure $\CONNSF(G^H)$
 with the deletion of the edge $e'$. We check whether $x$ and $y$ still belong to the same connected component of $\hat G^H$. If this is no longer the case, then the connected component to which both $x$ and $y$ belonged (that we denote by $C$), splits into two connected components, that we denote by $C_1$ and $C_2$. We check, in $O(\min\set{|C_1|,|C_2|})$ time, whether $|C_1|\leq |C_2|$, using the data structure $\CONNSF(G^H)$. Assume w.l.o.g. that this indeed holds (otherwise we switch between $C_1$ and $C_2$). We then replace $v_C$ with two vertices $v_{C_1}$ and $v_{C_2}$ in $\hat G^L$, in time $O(|C_1|)$, as follows. Using data structure $\CONNSF(G^H)$, we obtain a list of all vertices that belong to $C_1$. We create a new vertex $v_{C_1}$ in $\hat G^L$, which connects, with edges of length $1/4$, to every regular vertex in $C_1$. Additionally, we rename $v_{C}$ as $v_{C_2}$, and delete edges connecting $v_{C_2}$ to vertices of $C_1$. Lastly, for every $\EST$ $T_i$ that we maintain, with $v_{C}\in V(T_i)$, we run procedure $\splitsupernode(T_i,v_C,C_1,C_2)$.  Our algorithm will ensure that each vertex in the graph $\hgl$ belongs to at least one tree $T_i$. Since the processing time of $\splitsupernode(T_i,v_C,C_1,C_2)$ is at least $\Omega(|C_1|)$, we can charge the time needed to update the graph $\hat G^L$ due to the splitting of $C$ to the running time taken by the procedures  $\splitsupernode(T_i,v_C,C_1,C_2)$, without increasing their asymptotic running time.
 
 This completes the description of the algorithm, except that we need to show how we decide which centers to open or move. 
 The total update time of the algorithm can be asymptotically bounded by the total update time of the \LCD data structure and the total time needed to maintain all \ESTs $T_i$, which we analyze later.
 The following lemma will be useful for us.
 










\begin{lemma}\label{lem: path translation}
        There is a randomized algorithm, that, given any simple path $P$ in graph $\hat G^L$, whose endpoints, denoted by $x$ and $y$, are regular vertices, and whose length is denoted by $\ell$, computes a path $P^*$ of length at most $\ell+\eps D/8$ in the original graph $G$, connecting $x$ to $y$. The expected running time of the algorithm is $O(n\poly\log n)$.
\end{lemma}
\begin{proof}
We show how to transform the path $P$ into a path $P^*$ in the original graph $G$, connecting $x$ to $y$.


Let $v_{C_1},\ldots,v_{C_q}$ be all special vertices that appear on the path $P$. For $1\leq j\leq q$, let $w_j$ be the regular vertex preceding $v_{C_j}$ on $P$, and let $w'_j$ be the regular vertex following $v_{C_j}$ on $P$. Denote $n_j=|V(C_j)|$. For each $1\leq j\leq q$, we run the query $\shortpath(C_j,w_j,w'_j)$ in the data structure for graph $G^H$ maintained by Theorem~\ref{thm: responding to short-paths queries in heavy graph}, to obtain a path $Q_j$, connecting $w_j$ to $w'_j$ in $C_j$,  that contains at most
$\frac{n_j\alpha }{\tau}=\frac{n_j\eps D}{8n}$ vertices,  in expected time $O(n_j\poly\log n)$. %

We obtain the final path $P^*$, by replacing, for each $1\leq j\leq q$, the vertex $v_{C_j}$ of $P$ with the path $Q_j$ (excluding its endpoints). Let $\qset=\set{Q_i\mid 1\leq i\leq q}$ be the set of the resulting paths. The total length of all paths in $\qset$ is then bounded by $\sum_{j=1}^q\frac{\eps n_j D}{8n}\leq \frac{\eps D}{8}$ (since the path $P$ is simple, and so all connected components $C_j$ are distinct). 

Finally, we bound the total expected running time of the algorithm. Each query $\shortpath(C_j,w_j,w'_j)$ is processed in expected time $O(n_j\poly\log n)$.
Since all components $C_j$ are disjoint, $\sum_{j=1}^qn_j\leq n$, and so the total expected running time of the algorithm is $O(n\poly\log n)$.
\end{proof}


\begin{definition}
We say that a connected component $\hat C$ of $\hat G^L$ is \emph{small} if it contains at most $D/8$ regular vertices. 
\end{definition}



\begin{observation}\label{obs: connected components translation}
        Let $\hat C$ be a connected component of $\hgl$. Then there is a connected component $C$ of $G$, such that the vertices of $C$ are precisely all regular vertices of $\hgl$.
\end{observation}
\begin{proof}
        It is enough to show that for every pair $x,y$ of regular vertices in $\hgl$, there is a path connecting $x$ to $y$ in $\hgl$ iff there is a path connecting them in $G$. Let $x,y$ be any pair of regular vertices in $\hgl$. First, if there is a path $P$ connecting $x$ to $y$ in $\hgl$, then, from Lemma~\ref{lem: path translation}, there is a path $P'$, connecting $x$ to $y$ in $G$. Assume now that there is a path $P'$ connecting $x$ to $y$ in $G$. Let $w,w'$ be  a consecutive pair of vertices on $P'$, such that the edge $(w,w')$ does not lie in $G^L$. Then both $w$ and $w'$ have virtual degree at least $\tau$, and so the edge $(w,w')$ lies in the heavy graph $G^H$. In particular, $w$ and $w'$ lie in the same connected component of $G^H$, so there is some supernode in $\hgl$ to which both $w$ and $w'$ are connected. Therefore, we can transform $P'$ into a path $P$ in $\hgl$, connecting $x$ to $y$.
\end{proof}

\begin{corollary}\label{cor: small components}
        If $\hat C$ is a small connected component of $\hgl$, then there is a connected component $C$ of $G$, whose vertices are all regular vertices of $\hat C$, such that $|V(C)|<D$.
        \end{corollary}

Note that if $\hat C$ is a small connected component, then it will remain so until the end of the algorithm, or it will be split into a number of small connected components.






Recall that a vertex $u\in V(\hat G^L)$ is {covered} by a center $s_i$ iff $\dist_{\hgl}(u_i,u)\leq R^c$. We maintain 
the following invariant:

\begin{properties}{I}
        \item Throughout the algorithm, every vertex of $\hat G^L$ that does not lie in a small connected component of $\hat G^L$ is covered by some center in $S$.\label{Invariant: every vertex is covered}
\end{properties}


We now proceed as follows. We first provide an algorithm for responding to shortest-path query. 
We then complete the description of the center-moving data structure and analyze the total update time.

\subsubsection{Responding to Queries}

\paragraph{Responding to $\pathquery_D(x,y)$.}
Recall that we are guaranteed that $x$ and $y$ lie in the same connected component of $G$. Our goal is to either correctly establishes that $\dist_G(x,y)>2D$, or to correctly establishes that both $x$ and $y$ lie in a connected component of $G$ containing fewer than $D$ vertices, or to return a path connecting $x$ to $y$, of length at most $8D$. Moreover, if $D\leq \dist(x,y)\leq 2D$, then we need to return a path  from $x$ to $y$ of length at most $(1+\eps)\dist(x,y)$.

Note that, from Invariant~(\ref{Invariant: every vertex is covered}) either $x$ lies in a small connected component of $\hgl$, or there is some center $s_i\in S$ that covers $x$. Since we maintain, together with $x$, a list of all centers that cover it, together with pointers to them, we can, in time $O(1)$, either find a center $s_i$ that covers $x$, or correctly establish that no center covers $x$, so it lies in a small connected component of $\hgl$. In the latter case, from Corollary~\ref{cor: small components}, we know that both $x$ and $y$ lie in a connected component of $G$ containing at most $D$ vertices. We terminate the algorithm and report this.


 Assume now that we obtain a center $s_i$ that covers $x$.  Recall that $\dist_{\hat G^L}(x,u_i)\leq R^c=\eps D/4$ must hold. Notice that, from Observation~\ref{obs: distances in G and light graph for APSP}, $\dist_{\hat G^L}(y,u_i)\leq \dist_{\hat G^L}(y,x)+\dist_{\hat G^L}(x,u_i)\leq \dist_G(x,y)+\dist_{\hat G^L}(x,u_i)\leq \dist_G(x,y)+R^c$. In particular, if $\dist_G(x,y)\leq 2D$, then $\dist_{\hat G^L}(y,u_i)\leq 2D+R^c\leq 4D$, and therefore $y$ must lie in the tree $T_i$.

We check whether $y\in T_i$ using the data structures that we maintain. If this is not the case, then we report that $\dist_G(x,y)>2D$ and terminate the algorithm. Assume now that $y\in T_i$. We compute a simple path $P$, connecting $x$ to $y$ in $\hgl$, of length at most $\dist_{\hgl}(x,u_i)+\dist_{\hgl}(y,u_i)$, as follows. We traverse the paths connecting $x$ and $y$ to $u_i$ in the tree $T_i$ simultaneously, looking for a vertex $w$ with largest $\dist(u_i,w)$ that lies on both paths. It is easy to verify that the resulting path connecting $x$ to $y$ via $w$ is a simple path of length at most $\dist_{\hgl}(x,u_i)+\dist_{\hgl}(y,u_i)$, and that we can find it in time $O(n)$. Let $\ell$ denote the length of $P$.
We then use Lemma~\ref{lem: path translation} to turn it into a path $P^*$, connecting $x$ to $y$ in graph $G$, such that the length of $P^*$ is at most $\ell+\eps D/8$, in expected time $O(n\poly\log n)$. 
From the above discussion, if $D\leq \dist_G(x,y)\leq 2D$, then $\ell\leq \dist_G(x,y)+2R^c\leq\dist_G(x,y)+\eps D/2$, and the length of $P^*$ is bounded by $\ell+\eps D/8\leq \dist_G(x,y)+\eps D\leq (1+\eps)\dist_G(x,y)$.  The total expected time to compute a response to the query is $\tilde O(n)$.


\paragraph{Responding to $\distquery_D(x,y)$.}
Assume that we are given a pair $x,y$ of vertices of $G$, that lie in the same connected component of $G$. The algorithm for responding to $\distquery_D(x,y)$ is similar to that for responding to $\pathquery_D(x,y)$, except that we do not need to return the path itself.
As before, in time $O(1)$, we either find a center $s_i$ that covers $x$, or correctly establish that no center covers $x$, so it lies in a small connected component of $\hgl$. In the latter case, since $x$ and $y$ lie in the same connected component of $G$, we are guaranteed that $\dist_G(x,y)<D$. We terminate the algorithm and report this. Assume now that we obtain a center $s_i$ that covers $x$. We check, in time $O(1)$,  whether $y\in T_i$ using the data structures that we maintain. If this is not the case, then we are guaranteed that $\dist_G(x,y)>2D$. We terminate the algorithm and report this. Assume now that $y\in T_i$. 
Let $\dist'(x,y)$ be the sum of the labels of $x$ and $y$ in the tree $T_i$. 
Clearly, we are guaranteed that $\dist'(x,y)\geq \dist_G(x,y)$. Moreover, if $D\leq \dist_G(x,y)\leq 2D$, then we are guaranteed that $\dist'(x,y)\leq (1+\eps)\dist_G(x,y)$. Therefore, if $\dist'(x,y)<D$, then we are guaranteed that $\dist_G(x,y)<D$, which is what the algorithm reports. If $\dist'(x,y)>(1+\eps)^2D$, then we are guaranteed that $\dist_G(x,y)\geq (1+\eps)D$, which is what the algorithm reports. Otherwise, we return $\dist'(x,y)$, and we are guaranteed that $\dist_G(x,y)\leq \dist'(x,y)\leq (1+\eps)\dist_G(x,y)$.
The running time of the algorithm is $O(1)$.



\subsubsection{Maintaining the Center-Cover Data Structure}
Our center-cover data structure is very similar to that of~\cite{henzinger16}. We maintain a set $S$ of \emph{centers}, and for each center $s_i\in S$, we maintain a \emph{location} $u_i\in V(\hat G^L)$ of the center $s_i$, together with the \EST $T_i$ from Theorem~\ref{thm: maintain a single ES tree}. 
The data structure performs the following update operations:

\begin{itemize}
        \item $\opencenter(s_i,u_i)$: add a new center $s_i$ to $S$ with location $u_i$; initialize the data structure $T_i$ from Theorem~\ref{thm: maintain a single ES tree}; and
        
        \item $\movecenter(s_i,u_i,u'_i)$: move center $s_i$ from location $u_i$ to $u'_i$. In order to do so, we stop maintaining the tree $\EST(\hat G^L,u_i,R^d)$, and instead initialize the data structure for tree $\EST(\hat G^L,u'_i,R^d)$, using Theorem~\ref{thm: maintain a single ES tree}; the new tree becomes $T_i$.
\end{itemize}


We note that our algorithm never ``closes'' a center. Once a center is opened it remains so, though its location may move from vertex to vertex. 

Our algorithm maintains invariant~(\ref{Invariant: every vertex is covered}), to ensure that every vertex of $\hat G^L$ is covered by some center, except if it belongs to a small connected component. At the beginning of the algorithm, we spend time $O(|E(\hgl)|)=O(n\tau)$ to identify all connected components of $\hgl$, and all vertices that lie in small and large connected components. We mark every vertex as uncovered.
We initialize $S=\emptyset$, and then iterate, as long as there is some vertex $u\in G^L$ that does not lie in a small connected component and is not covered by the current centers. In every iteration, we select any such vertex $u$, and create a new center $s_i$, that is located at $u$, by employing the $\opencenter(s_i,u)$ operation. We then add $s_i$ to $S$. Note that the the algorithm that constructs the resulting tree $T_i$ from Theorem~\ref{thm: maintain a single ES tree} also marks all vertices that are covered by the new center $s_i$.

 Once we complete this initialization, every vertex of $G^L$ that lies in a large connected component is covered by some center. As the algorithm progresses, some vertex may stop being covered by the centers. This can happen in two cases: (i) if some edge is deleted from $\hat G^L$ as part of the edge-deletion sequence of the algorithm; we refer to such deletions as type-1 deletions; and (ii) if some supernode $v_C$ is split into $v_{C_1}$ and $v_{C_2}$, with $|C_1|\leq |C_2|$. Note that, in the latter case, we implement the split in two steps: in the first step, we insert a new vertex $v_{C_1}$ and connect it to the vertices of $C_1$; in the second step, we delete edges connecting $v_{C_2}$ to the vertices of $C_1$; we refer to these deletions as type-2 deletions. Each of these resulting deletions of edges may cause some vertex $x$ of $\hat G^L$ to become un-covered.

In general, whenever some vertex $u$ of $V(\hgl)$ that does not lie in a small connected component stops being covered by the centers, we open a new center at $u$, using procedure $\opencenter(s_i,u)$, with one exception. Consider the iteration when vertex $u$ stopped being covered, and let $e=(x,y)$ be the edge that was deleted in this iteration (note that $e$ may have been a type-1 or a type-2 deletion). Assume that $e$ belonged to some tree $T_i$, and let $\hat C$ be the connected component of $\hgl$ in which $T_i$ lies. Assume further that, as the result of the deletion of $e$, $\hat C$ decomposes into a small connected component $\hat C_1$, containing $u_i$, and a large connected component $\hat C_2$. Assume w.l.o.g. that $x\in \hat C_1$ and $y\in \hat C_2$. We then move the center $s_i$ from its current location $u_i$ to $y$. If, even after this move, some vertex $u$ that does not lie in a small connected component remains uncovered, we use operations $\opencenter(s_{i'},u)$ to ensure that all such vertices are covered. We emphasize that, if $\hat C_2$ is a small connected component, then we do not move $s_i$, and, from that point onward, $s_i$ will never be moved.


In order to identify when we need to move a center, recall that whenever an edge $e=(x,y)$ is deleted from $\hgl$, for each tree $T_i$ containing both $x$ and $y$, we run procedure $\deledge(T_i,e)$ (if $e$ is deleted as part of $\splitsupernode(T_i,v_C,C_1,C_2)$ operation, then this operation calls $\deledge(T_i,e)$ internally). Procedure $\deledge(T_i,e)$ consists of two steps. In the first step, it identifies a set $U$ of vertices, whose distance from $u_i$ has increased. This is done in time $\sum_{u\in U}\deg_{\hgl}(u)+O(1)\leq O(|E(\hgl)|)$. If, as the result of the deletion of $e$, the connected component $\hat C$ that contained $T_i$ decomposes into two connected components, the algorithm will discover at this step that none of the vertices of $U$ has a neighbor that is currently attached to $T_i$. 
If we denote by $\hat C$ the original connected component containing $T_i$, by $\hat C_1$ the new connected component (obtained after the deletion of $e$) containing $u_i$, and by $\hat C_2$ the new connected component containing the remainder of $\hat C$, then all vertices that are still attached to $T_i$ are contained in $\hat C_1$, and all vertices of $U$ are contained in $\hat C_2$. If there are fewer than $D/8$ regular vertices that are still attached to $T_i$ (something that we can check by exploring $T_i$ for $O(D)$ steps), then we are guaranteed that $\hat C_1$ is a small connected component (since the tree $T_i$ goes up to distance $4D$, and all edges have lenghts at most $1$, if $T_i$ has fewer than $D/8$ regular vertices, then its diameter is less than $D/4$, and so $T_i$ contains all vertices of the connected component in which $u_i$ lies). In this case, we check whether $U$ contains at least $D/8$ regular vertices. If this is not the case, then, from the same argument as before, the connected component $\hat C_2$ must be a small one. If we have established that $\hat C_1$ is a small connected component and $\hat C_2$ is a large connected component, then we move the center $s_i$ from $u_i$ to the endpoint $y$ of $e$ that lies in $\hat C_2$, using procedure $\movecenter(s_i,u_i,y)$.  The following theorem will be used to bound the change in the potential $\Psii$ due to the move of the center; note that we compare the potential $\Psii$ from before $e$ was deleted to the potential right after the center $s_i$ was moved.



\begin{claim}\label{claim: potential change due to move center}
        If $\movecenter(s_i,u_i,u'_i)$ is executed, then $\Psii$ increases by at most $O(\dist_{\hat G^L}(u_i,u'_i)\cdot n^2\poly\log n/(\eps D))$.
\end{claim}
\begin{proof}
        In order to prove the claim, it is enough to prove that, if $u_i$ and $u'_i$ are connected with an edge in $\hgl$, that is, $\dist_{\hgl}(u,u')=1$, then $\movecenter(s_i,u_i,u'_i)$ increases $\Psii$ by at most $O(n^2\poly\log n/(\eps D))$.
        
        We bound the increase in $\psii(u)$ for every vertex $u\in V(\hgl)$ separately. Consider any vertex $u\in V(\hgl)$. Assume first that $u$ was a vertex of $T_i$ before operation $\movecenter(s_i,u_i,u'_i)$ (that is, $u$ belonged to $T_i$ before the deletion of the edge $e$ that has triggered the $\movecenter$ operation). Since $T_i$ is a shortest-path tree, then $\dist_{\hgl}(u,u_i)\leq \dist_{\hgl}(u,u'_i)+1$. Therefore, if we denote by $\delta(u)$ the value $\delta_{s_i}(u)$ before the move, and by $\delta'(u)$ the value $\delta_{s_i}(u)$ after the move, then $\delta'(u)\leq \delta(u)+1$. If $u$ is a regular vertex, then $\psii(u)$ increases by at most $O(\deg_{\hgl}(u)+\tau)$, and if $u$ is a supernode, $u=v_C$, then $\psi_i(u)$ increases by at most $O(|C|\log^2|C|)$.
        
        Assume now that $u$ did not belong to $T_i$ before operation $\movecenter(s_i,u_i,u'_i)$, so $\psii(u)$ was $0$ before the operation, and $\dist(u_i,u)>R^d$. If $u$ does not belong to $T_i$ after the operation, then $\psii(u)$ remains $0$. Assume now that $u$ belongs to $T_i$ after the operation. Then $\dist(u_i',u)\geq R^d-1$ must hold, and so the new value $\delta_{s_i}(u)\leq 1$. The increase in $\psii(u)$ is then bounded as before: it is at most $O(\deg_{\hgl}(u)+\tau)$ if $u$ is a regular vertex, and at most $O(|C|\log^2|C|)$ if $u=v_C$ is a supernode. Overall, the total contribution of the regular vertices to the increase in the potential is bounded by $O(|E(\hgl)|+n\tau)=O(n\tau)=O(n^2\poly\log n/(\eps D))$, since $\tau=8n\alpha/(\eps D)$ and $\alpha=\poly\log n$, and the total contribution of the supernodes to the increase in the potential is bounded by $O(n\log^2n)$. The total increase in $\Psii$ is then bounded by $O(n^2\poly\log n/(\eps D))$.
\end{proof}




The running time for both operations $\opencenter(s_i,u_i)$ and $\movecenter(s_i,u_i,u'_i)$ is bounded by $O(|E(G^L)|)=O(n\tau)=O(n^2\poly\log n/(\eps D))$. Note that following operation $\opencenter(s_i,u_i)$, the total potential $\Psi$ increases by $\Psii\leq O(n^2\poly\log n/\eps)$, as discussed above. %





We analyze the running time of the algorithm in the following lemma.

\begin{lemma}\label{lem: running time}
        Assume that, over the course of the algorithm, at most $O(n/(\eps D))$ centers are opened, and the total distance that the centers are moved is bounded by $O(n)$. Then the total expected update time of the algorithm is at most $ O(n^{3}\pln/(D\eps^2))$.
\end{lemma}

\begin{proof}
Recall that for each center that we open, we spend running time $O(n^2\poly\log n/(\eps D))$ on the opening operation, and the total potential $\Psi$ increases by at most $O(n^2\poly\log n/\eps)$. 
        If at most $O(n/(\eps D))$ centers are opened, then the total time spent on $\opencenter$ operations, together with the total increase in the potential due to the opening of centers is bounded by:
        
        
        \[ O\left(\frac{n^2\poly\log n}{\eps }\cdot \frac{n}{\eps D}\right )=O\left (\frac{n^3\poly\log n}{\eps^2 D}\right ).\]
        
        
        If the total distance that the centers are moved is bounded by $O(n)$, then the total increase in the potential $\Psi$ due to the $\movecenter$ operations is bounded by $O(n^3\poly\log n/(\eps D))$. Additionally, each $\movecenter$ operation takes time $O(|E(\hgl)|)=O(n\tau)=O(n^2/(\eps D))$ to execute, and the total number of such operations is bounded by $O(n)$. Therefore, the total running time spent on $\movecenter$ operations, and the total increase in the potential due to the $\movecenter$ operation is bounded by $O(n^3\poly\log n/(\eps^2D))$.
        
        Note that, from Theorem~\ref{thm: maintain a single ES tree}, the total update time spent on all update operations of each tree $T_i$ is bounded by the decrease in the potential $\Psii$ due to the update operation, except that we pay an additional $O(1)$ for each deletion of an edge with both endpoints in $T_i$. The total number of edges ever present in $\hgl$ is bounded by $O(n\tau)+O(n\log n)=O(n^2\log n/(\eps D))$, and each such edge may need to be deleted from at most $O(n/(\eps D))$ trees $T_i$. Therefore, this total additional time due to edge deletions is bounded by $O(n^3\poly\log n/(\eps^2D^2))$. 
        
        Lastly, the total expected running time for maintaing the data structures $\CONNSF(G^H)$ and $\LCD$ are both $\tilde O(n^2)$. Therefore, the total expected running time of the algorithm is $O(n^3\poly\log n/(\eps^2D))$. 
        \end{proof}


It now only remains to show that the above algorithm indeed opens at most $O(n/(\eps D))$ centers,  and that the centers are moved at most distance $O(n)$ in total. This part is very similar to the analysis of the center-cover data structure of~\cite{henzinger16}. Throughout the algorithm, for every center $s_i\in S$, we maintain a \emph{witness set} $W_i$ of at least $R^c/16$ regular vertices of $\hat G^L$, such that for $i\neq j$, $W_i\cap W_j=\emptyset$. Since $\hgl$ contains $n$ regular vertices, and $R^c=\eps D/4$, this will ensure that the total number of all opened centers is at most $O(n/(\eps D)$. Moreover, we will ensure that, whenever a center $s_i$ is moved from $u_i$ to $u'_i$, then all regular vertices that lie on the shortest path from $u_i$ to $u'_i$ are added to $W_i$ and remain there until the end of the algorithm. Since all witness sets $W_i$ are disjoint, this will ensure that the total distance that the centers have moved is at most $O(n)$.

Each witness set $W_i$ is in turn partitioned into two subsets: set $W'_i$ of vertices that \emph{belong} to $s_i$, and set $W''_i$ of vertices that are \emph{borrowed} by $s_i$. All vertices in $W'_i$ lie in small connected components of $\hat G^L$, and set $W''_i$ contains all regular vertices lying at distance at most $\max\set{0,R^c/8-|W'_i|}$ from $u_i$ in $\hgl$. 

Notice that, when we execute operation $\opencenter(s_i,u_i)$, then vertex $u_i$ is not covered by any other vertex and does not lie in a small connected component of $\hgl$. Therefore, if we let $W_i$ be the set of all regular vertices lying at distance at most $R^c/8$ from $u_i$ in $\hgl$, then $W_i$ is guaranteed to be disjoint from all other sets $W_j$ for $s_j\in S$. We are also guaranteed that $W_i$ contains at least $R^c/16$ regular vertices, since the connected component of $\hgl$ to which $u_i$ belongs is not small. We set $W'_i=\emptyset$ and $W''_i=W_i$. As the algorithm progresses, set $W_i$ may evolve, but it will always be contained in the original set $W_i$, and it will always contain at least $R^c/16$ regular vertices.

Next, we consider the execution of procedure $\movecenter(s_i,u_i,u'_i)$. Recall that this procedure is executed if, as the result of the deletion of some edge $e=(x,y)$ from $\hgl$, the connected component $\hat C$ of $\hgl$ that contained $T_i$ before the deletion, splits into two connected components, $\hat C_1$ and $\hat C_2$, such that, if we denote by $\hat C_1$ the component containing both $x$ and $u_i$, then  $\hat C_1$ is a small connected component, and $\hat C_2$ is a large connected component.

Recall that procedure $\movecenter$ moves the center $s_i$ from its current location $u_i$ to the new location $y$, which is the endpoint of $e$ lying in $\hat C_2$. We add all regular vertices of $\hat C_1$ to $W'_i$, and we let $W''_i$ contain all regular vertices that lie within distance at most $\max\set{0,R^c/8-|W'_i|}$ from $y$ in the new graph $\hgl$ obtained after the deletion of $e$. Notice that all regular vertices on the shortest path from $u_i$ to $y$ now lie in $W'$, and that the new set $W''_i$ is contained in the original set $W''_i$. Moreover, since the component $\hat C_2$ is large, set $W''$ must contain at least $\max\set{0,R^c/8-|W'_i|}$ vertices. We set $W_i=W'_i\cup W''_i$. Notice that $W_i$ still contains at least $R^c/16$ regular vertices. 

Lastly, consider some iteration in which an edge $e=(x,y)$ of $T_i$ is deleted, such that $\hat C$ is a large connected component at the beginning of the iteration, and both $\hat C_1$ and $\hat C_2$ are small connected components at the end of the iteration. From this point onward we will never move $s_i$, and we will never open centers at vertices of $\hat C$. 
Notice that all vertices of $W_i$ lie in $\hat C_1\cup \hat C_2$. We do not change the set $W_i$ from this point onward. Since $W_i$ is disjoint from all other current witness sets, and since we will never open another center in $\hat C_1\cup \hat C_2$, witness set $W_i$ will remain disjoint from all other witness sets.

This guarantees that, throughout the algorithm, all witness sets $\set{W_i}_{s_i\in S}$ are disjoint; each set $W_i$ contains at least $R^c/16$ regular vertices, and, whenever $\movecenter(s_i,u_i,u'_i)$ is called, all regular vertices on the shortest path from $u_i$ to $u'_i$ are added to $W_i$ and remain there. Therefore, the total number of centers that we ever open is bounded by $O(n/R^c)=O(n/(\eps D))$, and the total distance traveled by the centers is bounded by $O(n)$.





\subsection{The Small-Distance Regime}\label{APSP: small dist}
The goal of this section is to prove Theorem~\ref{thm: main for APSP w distance bound: small dist}. We assume that we are given a parameter $k\geq 1$ and a distance scale $D$. We set $\Delta=n^{1/k}$. We define the virtual degrees of vertices with respect to this value of $\Delta$.
Recall that, if $\dmax$ is the maximum vertex degree in $G$, then $r$ is the smallest integer, such that $\Delta^{r-1}>\dmax$ (in particular, $r\leq k+1$), and for all $1\leq j\leq r$, $h_j=\Delta^{r-j}$.

 We maintain the \LCD data structure from Section~\ref{sec: LCD}, with the parameter $\Delta$ and $q$. The data structure maintains a partition of vertices into layers 
$\Lambda_1,\ldots,\Lambda_{r}$ where $\Lambda_{i}$ contains all vertices with virtual degree $h_j$. In addition to the $\LCD$ data structure, our algorithm will maintain, for every index $1\leq j\leq r$, a collection $\tset_j$ of \ESTs associated with layer $j$. For each $1\leq j\leq r$, we define two distance parameter: parameter $R^d_j$ is the depth of the \ESTs in $\tset_j$, and $R^c_j$ is their \emph{covering radius} (that is, a vertex $v$ whose distance from the root of a tree $T\in \tset_j$ is at most $R^c_j+1$ will be considered covered by that tree). 

Let $\alpha= \log^{O(q)}n$ be such that the length of the paths returns by the $\shortkpath$ and $\tocore$ queries from the $\lcd$ data structure \Cref{thm:LCD} is always at most $\alpha/2$. 
We are now ready to define the distance and the covering radii.
For $1\leq j\leq r$, we have
$$R^d_j=4^{r-j+2}D+r\alpha^{r-j+2} \text{ and } R^c_j=R^d_j-2D.$$

Note that for all $j$, $R^d_j\leq 4^{k+1}D+\alpha^{k+1}=O(D\cdot \log^{O(qk)}n)$.
We now describe the data structures that we maintain for each layer $\Lambda_j$.

\label{APSP: small-distance dense}
Throughout this subsection, we fix some index $1\leq j\leq r$. We will use an auxiliary graph $Z_j$, associated with layer $j$, that is defined as follows. The set of vertices is $V(Z_j)=V(G)$. The set of edges contains, for every vertex $v\in V(G)$ with $\td_G(v)\leq  h_j$, all edges incident to $v$ in $G$. Note that, from \Cref{claim:bound edge} and from the fact that the virtual degrees $h_j$ form a geometrically decreasing sequence, the total number of edges of $G$ that ever belong to $Z_j$ is bounded by  $O(nh_j\Delta)$.

**TO\ EDIT FROM\ HERE**

\begin{definition}
        We say that a vertex $v\in \Lambda_j$ is \emph{happy} iff there is a vertex $u\in \Lambda_1\cup\cdots\cup \Lambda_{j-1}$, such that $\dist_G(v,u)\leq R^d_j$.
\end{definition}

Informally, a vertex from layer $j$ is happy iff there is some vertex from layers $\Lambda_1\cup\cdots\cup \Lambda_{j-1}$, that is close enough to it, that is, within distance $R^d_j$ - the depth radius for layer $j$. Recall that virtual degrees of vertices may only decrease over the course of the algorithm, and that set $\Lambda_j$ contains all vertices with virtual degree $h_j$. Therefore, if a vertex $v\in \Lambda_j$ is not happy (that is, it is far from all vertices in $\Lambda_1,\ldots,\Lambda_{j-1}$), it will remain so as long as it remains in $\Lambda_j$. If $v$ is a happy vertex, then it may become unhappy at some later point.

We will maintain a collection $\tset_j$ of \ESTs, where each such tree $T$ is rooted at some core of $\fset_j$. Next, we define when a core is eligible to become a root of such a tree. We will only maintain trees from eligible cores.

\begin{definition}
        A core $K\in \fset_j$ is \emph{eligible} iff every vertex of $S^K$ is unhappy.
\end{definition}

Consider some level-$j$ phase. Note that if, at any point during the phase, some core $K$ becomes eligible, then it will remain eligible for the remainder of the phase. Next, we define several data structures for layer $j$. The first data structure will allow us to determine, dynamically, which vertices of $\Lambda_j$ are happy. The second data structure will allow us to determine which cores are eligible. The third data structure is the collection of $\tset_j$ of \ESTs rooted at the eligible cores. Finally, we will use a coverage data structure to keep track, for every vertex $v$, of all trees of $\tset_j$ that contain $v$, and all trees of $\tset_j$ that cover $v$. We note that some of these data structures (such as the trees in $\tset_j$) are recomputed from scratch in every level-$j$ phase.


\subsubsection{Determining Happiness}\label{subsub: DS: happiness}
We construct a data structure that allows us to determine, dynamically, which vertices of $\Lambda_j$ are happy. In order to do so, we utilize the graph $Z_j$ that we have defined above. Recall that  $V(Z_j)=V(G)$, and $E(Z_j)$ contains, for every vertex $v\in V(G)$ with $\td_G(v)\leq h_j$, all edges incident to $v$ in $G$. Recall also that the total number of edges of $G$ that are ever present in $Z_j$ is bounded by $ O(nh_j\Delta)$.

We construct a graph $Z'_j$, by adding a source vertex $s$ to $Z_j$, and connecting $s$ to every vertex in $\Lambda_1,\ldots,\Lambda_{j-1}$. Notice that a vertex $v\in \Lambda_j$ is happy if and only if the distance from $s$ to $v$ in $Z'_j$ is at most $R^d_j+1$.

Our algorithm will maintain an \EST $\hat T_j$ in graph $Z'_j$, with $s$ as a source, and depth bound $R^d_j+1$, so $\hat T_j=\EST(Z'_j,s,R^d_j+1)$. Note that the tree will need to handle both edge deletions and edge insertions. Indeed, if, due to the deletion of an edge $e$ from $G$, the virtual degree of some vertex $v$ fell from $h_{j'}$ for $j'<j$ to $h_{j''}$ for $j''\geq j$, then we need to insert all edges that are incident to $v$ in $G$ into $Z'_j$.
We now describe how the tree $\hat T_j$ is maintained.

\paragraph{Initialization.} We compute the tree $\hat T_j$ from scratch at the beginning of the algorithm, right after Procedure $\PCL(j)$ is executed for the first time. The construction of the graph $Z'_j$ and the tree $\hat T_j$ takes total time proportional to the number of edges with at least one endpoint in $V(Z_j)$, which is bounded by  $O(nh_j\Delta)$.

\paragraph{Updates.} We now consider some iteration when some edge $e$ is deleted from graph $G$. We update the \LCD data structure with the deletion of the edge $e$. As the result, we may obtain a collection $X$ of vertices of $G$, such that, for each $x\in X$, the virtual degree of $x$ was greater than $h_j$ before the deletion of $e$, and became at most $h_j$ after the deletion of $e$. For each such vertex $x\in X$, let $E(x)$ be the set of edges that are incident to $x$ in $G$ and do not currently belong to $Z'_j$. Note that $E(x)$ is precisely the set of edges connecting $x$ to other vertices of $X$, or to vertices that currently lie in $\Lambda_1\cup\cdots\cup \Lambda_{j-1}$. We consider the edges in $\bigcup_{x\in X}E(x)$ one-by-one, and insert each such edge into $Z'_j$. We claim that for each such edge $e'=(x,y)$, the insertion of $e'$ into $Z'_j$ does not decrease the distance of any vertex from $s$. Indeed, observe that $x$ is currently connected to $s$ with an edge, and, from the above discussion, so is $y$. Therefore, the insertion of $e'$ does not decrease the distances of the vertices of $Z'_j$ from $s$, and so edge $e'$ can be inserted into the data structure $\hat T_j$ in a straightforward way, in time $O(1)$. Once all edges of  $\bigcup_{x\in X}E(x)$ are inserted into $\hat T_j$, we delete, for every vertex $x\in X$, the edge $(s,x)$ from $Z'_j$, and we update the data structure $\hat T_j$ accordingly. Since the total number of edges that are ever present in $Z'_j$ over the whole course of the algorithm is $O(nh_j\Delta)$, the total update time of the data structure, over the course of the algorithm, is $O(nh_j\Delta R^d_j)=
O(nh_j\Delta D\log^{O(k)}n)=O(n^2 D\log^{O(k)}n)$. If the deleted edge $e$ lies in $Z_j$, then we update the data structure $\hat T_j$ with its deletion.

\subsubsection{Determining Eligibility}\label{subsub: DS: eligibility}
In this subsection we describe a data structure that allows us to determine which cores of $\fset_j$ are eligible. Recall that the set $\fset_j$ is recomputed at the beginning of every level-$j$ phase; our data structure will also be recomputed then.

The data structure maintains  list $L_j$ of all eligible cores in $\fset_j$. For every core $K \in \fset_j$, it maintains a list $L_j(K)$ of all vertices of $S^k$ that are happy, and a counter $n_j^K$ for the number of such vertices. 

\paragraph{Initialization.} The data structure is initialized at the beginning of every level-$j$ phase, right after Procedure \CCD is executed. For every core $K$, we scan all vertices of $V(K)$ and use the tree $\hat T_j$ to determine whether $K$ is an eligible core, and if not, to initialize the list $L_j(K)$ of happy vertices of $V(K)$, and the counter $n_j^K$.

\paragraph{Updates.} We consider an iteration when some edge $e$ is deleted from $G$. We update the \LCD and the $\hat T_j$ data structures with this deletion. Note that, if $e\in E(K)$ for some core $K\in \fset_j$, then it is possible that some vertices of $S^K$ are deleted from the set $S^K$. If $K$ is not an eligible core, for each such vertex $v$, we check whether it is happy. If so, we delete it from $L_j(K)$, and update the counter $n_j^K$. Additionally, it is possible that some new vertices $u$ may become unhappy and deleted from the tree $\hat T_j$. Note that each such vertex $u$ may belong to at most one core $K\in \fset_j$. If $K$ is not an eligible core, and $u\in S^K$, then we delete $u$ from the list $L_j(K)$, and we update the counter $n_j^K$ accordingly. Finally, if, for some core $K$ that was not eligible before the deletion of $e$, the counter $n_j^K$ fell to $0$, then $K$ becomes eligible and is added to $L_j$. 

The running time needed to update this data structure for all $1\leq j\leq r'$ is asymptotically smaller than the running time of procedure \LCD and the running time needed to maintain the data structure  $\hat T_j$, and we charge it to them.


\subsubsection{The ES-Trees}\label{subsub: DS: trees}
We now describe the set $\tset_j$ of \ESTs that we maintain for layer $j$. 
Throughout the algorithm, for every eligible core $K\in \fset_j$, the algorithm maintains a data structure $T_j(K)$, that is defined as follows. Let $Z^K_j$ be the graph obtained from $Z_j$ by adding a source vertex $s(K)$, and connecting it to every vertex in $K$ with an edge. We let $T_j(K)$ be an \EST in graph $Z_j^K$, rooted at $s(K)$, with depth bound $R^d_j+1$, that is, $T_j(K)=\EST(Z_j^K,s(K),R^d_j+1)$. We then let $\tset_j$ be the set of all such trees $T_j(K)$ for all eligible cores $K\in \fset_j$. We now describe how we initialize and maintain these data structures.


\paragraph{Initialization.}
At the beginning of each level-$j$ phase, we identify all eligible cores using the data structure described above, and for each such eligible core $K$, we initialize the \EST $T_j(K)$. Over the course of the phase, whenever a new core $K\in \fset_j$ is added to a list $L_j$ of eligible cores, we initialize the tree $T_j(K)$. Note that, if a core $K$ becomes eligible, then it will continue to be so until the end of the current level-$j$ phase.

Observe that, since all cores in $\fset_j$ are disjoint, and since every core must contain at least $h'_j=\Omega(h_j/\poly\log n)$ vertices, the total number of trees in $\tset_j$ that we construct over the course of a phase is bounded by $n\poly\log n/h_j$.
Each such tree takes time $O(|E(Z_j)|+n)=O(nh_j\Delta)$ to construct.

\paragraph{Updates.}
We now fix some tree $T_j(K)$, and describe the updates that need to be done to the tree over the course of a level-$j$ phase. Consider an iteration when some edge $e$ is deleted from the graph $G$. We first update the deletion of $e$ in the \LCD data structure. Note that, as the result of the deletion of $e$, it is possible that some vertices that belonged to $S^K$ prior to the update, no longer belong to $S^K$. For each such vertex $x$, we simply delete the edge connecting the source $s(K)$ to $x$ in the  data structure $T_j(K)$. Additionally, if $e$ is an edge of some tree $T_j(K')$, then we update $T_j(K')$ to reflect its deletion. We claim that we will never need to insert any edges or vertices into the trees of $\tset_j$. Indeed, let  $T_j(K)\in \tset_j$ be any such tree. We only need to insert edges into graph $Z_j$ when the virtual degree of some vertex $y$, that was greater than $h_j$ before the deletion of the edge $e$, becomes at most $h_j$ after the deletion of $e$. Whenever this happens, we insert all edges that are incident to $y$ and do not currently belong to $Z_j$, into the graph $Z_j$. This is the only scenario when edges are inserted into $Z_j$. Notice however that, before the deletion of $e$, $K$ was an eligible core. Therefore, for every vertex $v\in S^K$, $\dist_G(v,y)>R_j^d$ held before the deletion of $e$. Therefore, $\dist_{Z_j^K}(s(K),y)>R_j^d$, and we do not need to insert $y$ or any edges that are adjacent to it into $T_j(K)$ in order to ensure that it remains a valid \EST in $Z_j^K$, with source $s(K)$ and depth bound $R^d_j+1$.

To summarize, over the course of a single level-$j$ phase, we may add at most $O(n\poly\log n/h_j)$ \ESTs to $\tset_j$. Each of these trees contains at most $O(n\Delta h_j)$ edges, and has depth bound $R^d_j$. Therefore, the total time needed to construct and to update each one of these trees is at most $O(n\Delta h_j R^d_j)$, and the total time spent on maintaining these trees over the course of the phase is $ O(n^2\Delta R^d_j\pln)=O(n^2\Delta D\log^{O(k)}n)$. From Observation~\ref{obs: num of phases}, the total number of level-$j$ phases is bounded by  $ O(n\Delta\pln/h_j)$. Therefore, altogether, the total time needed to maintain the data structure $\tset_j$ over the course of the entire algorithm is at most $O(n^3\Delta^2 D\log^{O(k)}n/h_j)$. Since the values $h_j$ form a geometrically decreasing sequence, and since $h_{r'}= \tau$,  the total time needed to maintain all data structures  $\set{\tset_j}_{j=1}^{r'}$ is at most ${O(n^3\Delta^2 D\log^{O(k)}n/\tau)}$. This also bounds the total time that we need in order to maintain the \LCD data structure, and the data structures from Sections~\ref{subsub: DS: happiness} and \ref{subsub: DS: eligibility}.


\subsubsection{Keeping Track of Coverage}
Fix a pair $1\leq j\leq j'\leq r'$ of indices. Let $v$ be a vertex of $\Lambda_{j'}$, and let $T_j(K)\in \tset_j$ be some tree. 
We say that $v$ is \emph{covered} by the tree $T_j(K)$ iff $v$ lies at distance at most $R_j^c+1$ from $s(K)$ in the tree $T_j(K)$. We say that $v$ is covered by $\tset_j$, iff it is covered by some tree in $T_j(K)\in \tset_j$.


In this subsection we describe the last data structure that we use for layer $\Lambda_j$, which allows us to quickly check which trees of $\tset_j$ cover a given vertex $v$, and to which trees it belongs. Additionally, we prove a lemma that shows that every vertex of $\Lambda_j$ is covered by some tree in $\tset_1\cup\cdots\cup\tset_j$. We start with describing the data structure.

Recall that the total number of cores that may belong to $\fset_j$ is bounded by $n/h'_j=O(n\poly\log n/h_j)$. Let $b_j$ denote this number. We will assume that the cores in $\fset_j$ are always indexed as $K_1,\ldots,K_{b'_j}$, where $b'_j\leq b_j$. For every vertex $v\in V(G)$, we maintain two arrays, $A^j_v$ and $B^j_v$, of length $b_j$ each. For all $1\leq i\leq b_j$, the entry $A^j_v[i]$ is $1$ if $v$ is a vertex of the tree $T_j(K_i)$, and it is $0$ if $b'_j<i$ (that is, we have fewer than $i$ cores in $\fset_j$), or $K_i$ is not an eligible core, or $v$ does not lie in the tree $T_j(K_i)$. If $A^j_v[i]=1$, then we also store a pointer from this array entry to the copy of $v$ in $T_j(K_i)$. Array $B^j_v$ is defined similarly, except that the value $B^j_v[i]$ is $1$ iff $v$ is covered by the tree $T_j(K_i)$, that is, the distance, in $Z^{K_i}_j$, from $s(K_i)$ to $v$ is at most $R^c_j+1$; equivalently, there is a vertex $u\in S^{K_i}$ such that $\dist_{Z_j}(u,v)\leq R^c_j$, and $K_i$ is an eligible core. At the beginning of every level-$j$ phase, we set all values in every array $A^j_v,B^j_v$ for $v\in V(G)$ to $0$. Whenever we initialize a new tree $T_j(K_i)$, we update the values $A^j_v[i]$ and $B^j_v[i]$ for all $v\in V(G)$. We then maintain these values up to date as the tree $T_j(K_i)$ is updated. Note that we have used the bound of $O(n\Delta h_jR^d_j)$ on the total update time for each such tree $T_j(K_i)$; the time needed to maintain the entries $A^j_v[i]$ and $B^j_v[i]$ is clearly bounded by this amount. It is easy to verify that the arrays $A^j_v$ and $B^j_v$ for all $v\in V(G)$ and $1\leq j\leq r'$ can be maintained without asymptotically increasing the total update time of the algorithm so far, which remains $O(n^3D\Delta^2\log^{O(k)}n/\tau)$.

\subsubsection{Every vertex is covered}

Following is the main lemma of this subsection.

\begin{lemma}\label{lem: coverage in layers}
        For all $1\leq j\leq r'$, every vertex $x\in \Lambda_j$ is covered by some tree $T\in \tset_1\cup\cdots\cup\tset_j$, and moreover, there is a tree $T=T_{j'}^K \in \tset_{j'}$, for some $j'\leq j$ that covers $x$, such that the distance, in $Z_{j'}^K$, from  $s(K)$ to $x$ is at most $R^c_{j'}-2D+1$.
\end{lemma}

\begin{proof}
        Fix some index $1\leq j\leq r'$, and some vertex $x\in \Lambda_j$. We will construct a non-empty sequence $K_1,K_2,\ldots,K_q$ of cores\footnote{This indexing of the cores is different from the indexing that we use within each set $\fset_j$ as described above; we abuse the notation here to avoid using cumbersome notation.}, such that, if we denote, for $1\leq a\leq q$, by $j_{a}$ the index of the layer to which $K_{{a}}$ belongs (that is, $K_{{a}}\in \fset_{j_{a}}$),  then the following hold:
        
        \begin{itemize}
                \item $j\geq j_1>j_2>\ldots>j_q$;
                \item there is a path $P(x)$ from $x$ to some vertex $v_1\in S^{K_1}$ of length at most $\alpha/2$, and for all $1\leq a<q$, there is a path $P_{a}$ from some vertex $v'_{a}\in S^{K_{a}}$ to some vertex $v_{a+1}\in S^{K_{a+1}}$, of length at most $\alpha/2+R^d_{j_a}$; moreover, paths $P(x),P_1,\ldots,P_{q-1}$ only contain vertices whose virtual degrees are at most $h_q$.
                \item all cores in the sequence are not eligible, except for the last core $K_q$, which is eligible.
        \end{itemize}
        
        In order to construct the sequence of cores, we use Claim~\ref{claim: find path procedure}
        to find a path $P(x)$ of length at most $\alpha/2$, connecting $x$ to some vertex $v_1\in \hat K_{j_1}$, for some index $j_1\leq j$, such that all vertices on the path have virtual degrees at most $h_{j_1}$. Therefore, there must be some core $K_1\in \fset_{j_1}$, such that $v_1\in S^{K_{j_1}}$. We add $K_1$ to our sequence. If $K_1$ is an eligible core, then we terminate the algorithm and return the sequence consisting of $K_1$ only. Otherwise, we continue to the next iteration.
        
        Assume now that we are given the core $K_{a}\in \fset_{j_{a}}$, such that $K_{a}$ is not eligible. 
        Then there is some index $\hat j<j_{a}$, and some vertex $u\in \Lambda_{\hat j}$, that prevented $K_{a}$ from being eligible; that is, for some vertex $v'_{a}\in S^{K_{a}}$ there is a path $P'$ of length at most $R^d_{a}$ from $v'_{a}$ to $u$. We can assume w.l.o.g. that all vertices on $P'$, except for the last one, have virtual degrees below $h_{\hat j}$, or we could make the path shorter. Using again Claim~\ref{claim: find path procedure}, there is a path $P(u)$ of length at most $\alpha/2$, connecting $u$ to some vertex $v_{a+1}$ of $\hat K_{j_{a+1}}$, for some $j_{a+1}\leq  \hat j < j_a$, such that every path on $P(u)$ has virtual degree at most $h_{j_{a+1}}$. Assume that $v_{a+1}\in S^{K_{a+1}}$ of some core $K_{a+1}\in \fset_{j_{a+1}}$. We add $K_{{a+1}}$ to our sequence, with the corresponding path $P_a$ that is a concatenation of $P'$ and $P(u)$. Observe that the length of $P_a$ is at most $\alpha/2+R^d_{j_a}$, and that it only contains vertices whose virtual degree is at most $h_{j_{a+1}}$. If $K_{{a+1}}$
        is an eligible core, we terminate the algorithm; otherwise we continue to the next iteration.
        
        Consider now the final sequence of cores $K_1,\ldots,K_q$ that we have constructed. For each $1\leq a\leq q$, we use Theorem~\ref{thm: short path in core} to conclude that there is a path $P'_a$ of length at most $\alpha/2$, connecting $v_a$ to $v'_a$. The path is contained in $K_a$, and so it only contains vertices of virtual degree $h_{j_a}$. By concatenating the paths of $P(x),P'_1,P_1,P'_2,P_2,\ldots,P_q$, we obtain a path $P^*$ that connects $x$ to a vertex of $K_q$. All vertices of $P^*$ have virtual degrees at most $h_{j_q}$, and so all edges and vertices of $P^*$ lie in the graph $Z_{j_q}$. Recall that $K_q$ is an eligible core of $\fset_{j_q}$, so there is a tree $T_{j_q}(K_q)\in \tset_{j_q}$ rooted at $s(K_q)$. If we show that the length of the path $P^*$ is bounded by $R^c_{j_q}-2D$, then this will prove the lemma.
        
        For simplicity, denote $j_{q}+1$ by $j'$ and denote $j_1$ by $j''$. Since, for all $1\leq j\leq r$, $R^d_j=4^{r'-j+2}D+r\alpha^{r'-j+2}$, we can bound the length of the path $P^*$ by:   
        \[\begin{split}
        \alpha q+\sum_{a=1}^{q-1}R^d_{j_a}&\leq \alpha (j''-j')+    R^d_{j''}+R^d_{j''+1}+\cdots+R^d_{j'} \\
        &=\alpha (j''-j')+\sum_{z=j'}^{j''}4^{r'-z+2}D+\sum_{z=j'}^{j}r\alpha^{r'-z+2}\\
        &=\alpha (j''-j')+D\cdot \frac{4^{r'-j'+3}-4^{r'-j''+2}}{3}+r\frac{\alpha^{r'-j'+3}-\alpha^{r'-j''+2}}{\alpha-1}\\
        &\leq r\alpha +\left(D\cdot 4^{r'-(j'-1)+2}+r\alpha^{r'-(j'-1)+2}\right )-(4D+\alpha r) \\
        &\leq R^d_{j'-1}-4D\\
        &\leq R^c_{j'-1}-2D.
        \end{split}  \]
        
        
        Recall that $j'=j_{q}+1$, and so $j'-1=j_q$. Therefore, we have shown that the length of the path $P^*$ is bounded by $R^c_{j_q}-D$ as required.
\end{proof} 



        
        
        
        \subsubsection{Responding to Queries}
        In this section we provide an algorithm for responding to queries $\pathquery_D(u,v)$ and $\distquery_D(u,v)$. 
        
        
        \paragraph{Responding to $\pathquery_D(u,v)$.}
        Recall that as part of the query, we are given a pair $u,v\in V(G)$ of vertices. The algorithm will either return an empty path, or a path  connecting $u$ to $v$ of length at most $2^k\cdot D+\log^{O(k)} n$, such that, if $D\leq \dist_G(u,b)\leq 2D$, then a non-empty path is always returned.
        
        The algorithm inspects the heap $H(u)$ of vertex $u$ to check whether $u$ is covered by any tree in $(\tset_1\cup\cdots\cup\tset_r)\cup \tset^L$. If this is not the case, then we return the empty path. Assume now that the heap $H(u)$ is not empty, and let $T$ be the tree with the smallest rank in $H(u)$, so $T$ must cover $u$. Using the arrays $A^1_v,\ldots,A^r_v,A^L_v$, we check whether $v$ belongs to the tree $T$. If this is not the case, then we return an empty path. Assume now that $v$ lies in the tree $T$, and let $\rank(T)=j$. We now consider two cases.
        
        Assume first that $j=r+1$, that is, $T\in \tset^L$, and assume that $T$ is the $i$th tree in $\tset^L$. Let $s$ denote the root of $T$. We use the entries $A^L_v[i],A^L_u[i]$ to reach the copies of $u$ and $v$ in the tree $T$. We then follow the paths connecting $u$ to $s$ and $v$ to $s$ in the tree $T$, to find the lowest common ancestor of $u$ and $v$ in the tree. By concatenating the two resulting paths together, we obtain a simple path connecting $u$ to $v$ in $G$, of length at most $2R^d_L$. We return the resulting path.
        
        Assume now that $j\leq r$, so $T\in \tset_j$. Assume that $T=T^{K_i}_j$ for some core $K_i\in \fset_j$. As before,  we use the entries $A^j_v[i],A^j_u[i]$ to reach the copies of $u$ and $v$ in the tree $T$. As before, we  follow the paths connecting $u$ to $s(K_i)$ and $v$ to $s(K_i)$ in the tree $T$, to find the lowest common ancestor of $u$ and $v$ in the tree, that we denote by $w$. If $w\neq s(K_i)$, then we have obtained a simple path connecting $u$ to $v$ in $G$, of length at most $2R^d_j$. Assume now that $w=s(K_i)$. Let $u'$ denote the penultimate vertex on the path $P_1$, connecting $u$ to $s(K_i)$ in $T$, and let $v'$ be the penultimate vertex on the path $P_2$, connecting $v$  to $s(K_i)$ in $T$. Note that $u',v'\in S^{K_i}$ must hold. We use  Theorem~\ref{thm: short path in core} to compute a  path $Q$ connecting $u'$ to $v'$, of length at most $\alpha/2$ in $K_i$, in expected time $O\left(\frac{|E(K_i)|\cdot \poly\log n}{h_j}\right )=O(\left(\frac{|E(H_j)|\cdot \poly\log n}{h_j}\right )=O(n\Delta\poly\log n)=\tilde O(n^{1+1/k})$.
        We return a path connecting $u$ to $v$ in $G$, obtained by concatenating $P_1,Q$, and $P_2$.
This completes the description of the algorithm. Notice that the expected running time is $\tilde O(n^{1+1/k})$. We use the following simple observation to bound the length of the returned path.

\begin{observation}\label{obs: path length}
        If the algorithm returns a non-empty path, then the path length is at most $2^{k+1}D+\log^{O(k)}n$.
\end{observation}

\begin{proof}
        Since $\Lambda_1=\emptyset$, the length of the path is bounded by $2R_2^d+\alpha/2\leq 2\cdot 4^{r'}D+r\alpha^{r'}+\alpha/2\leq 2^{2r'+1}D+\log^{O(k)}n$. It is now enough to show that $r'\leq k/2$. Recall that we have defined $r'$ such that $h_{r'}=\tau$. Since $h_{r'}=\Delta^{r-r'}$, and since $\tau\geq \sqrt{nD \Delta}\geq \sqrt{n \Delta}$, while $\Delta=n^{1/k}$, we get that:
        \[ \Delta^{r-r'}=n^{(r-r')/k}\geq n^{1/2+1/(2k)}. \]
        
        Therefore, $r-r'\geq k+1/2$. Since $r\leq k$ must hold (as $\dmax<n$), we get that $r'\leq k/2$.
\end{proof}

We complete the correctness proof with the following claim.

\begin{claim}\label{claim: query correctness}
        If $D\leq \dist_G(u,v)\leq 2D$, then the algorithm returns a non-empty path connecting $u$ to $v$.
\end{claim}

\begin{proof}
        Observe that the algorithm returns the empty path in two cases: (i) if $u$ is not covered by any tree; and (ii) if $v$ does not lie in the tree $T$ -- the tree of the smallest rank that covers $u$.
        
        If $u$ is not covered by any tree, then it must belong to a small and lonely connected component $C$ of $G^L$. If $v$ lies in the same connected component, then, from Observation~\ref{obs: small dont need centers}, $\dist(u,v)<D$. Otherwise, from Observation~\ref{obs: small and lonely CCs}, no path connects $u$ to $v$ in $G$. Therefore, if $D\leq \dist_G(u,v)\leq 2D$, then $u$ must be covered by some tree.
        
        Let $T$ be the tree in $H(u)$ that has the smallest rank. It now remains to show that $v$ also lies in $T$.
        
        
        Let $P$ be the shortest path connecting $u$ and $v$ in $G$, so that the length of $P$ is at most $2D$. Let $x$ be the vertex of $P$ with largest virtual degree, breaking ties arbitrarily. If $\td(x)<\tau$, then the whole path $P$ lies in the light graph $G^L$, and so all edges and vertices of $P$ lie in every graph $Z_j$, for $1\leq j\leq r$. We claim that in this case, every tree in $(\tset_1\cup\cdots\cup\tset_{r'})\cup \tset^L$ that covers $u$ must also contain $v$. Indeed, let $T'$ be any such tree. Assume first that $T'\in \tset^L$, and let $s$ be the root of the tree. Since $u$ is covered by $T$, $\dist_{G^L}(s,u)\leq R^c_L=2D$. Since path $P$ is contained in $G^L$, $\dist_{G^L}(u,v)\leq 2D$, and so $\dist_{G^L}(s,v)\leq 4D$. Since $R^d_L=4D$, vertex $v$ must lie in $T$.
        Assume now that $T\in \tset^j$ for some $1\leq j\leq r'$, and let $K\in \fset_j$ be the core such that $T=T_j(K)$. Since $u$ is covered by $T$, there is some vertex $y\in S^K$, such that $\dist_{Z_j}(y,u)\leq R^c_j$. But then, since $P\subseteq Z_j$, $\dist_{Z_j}(y,v)\leq \dist_{Z_j}(y,u)+\dist_{Z_j}(v,u)\leq R^c_j+2D\leq R^d_j$, so $v$ lies in $T$.
        
        
        It now remains to analyze the case where $\td(x)\geq \tau$. Assume that $\td(x)=h_{j'}$. Then all edges and vertices of $P$ lie in all graphs $Z_1,\ldots,Z_{j'}$. From Lemma~\ref{lem: coverage in layers}, there is an index $j''\leq j'$, and a tree $T'\in \tset_{j''}$, such that $T'$ covers $x$, and moreover, if we denote by $K'$ the core that serves as the root of $T'$, then the distance, in $Z_{j''}^{K'}$, from the root $s(K')$ of the tree $T'$ to $x$ is at most $R^c_{j''}-2D+1$. Since path $P$ is contained in $Z_{j''}$, the distance, in $Z_{j''}^{K'}$, from $s(K')$ to $u$ is at most $R^c_{j''}$, and so $u$ is covered by $T'$. Therefore, if $T$ is the tree of the smallest rank in $H(u)$, and the rank of $T$ is $j$, then 
        $j\leq j''\leq j'$ must hold, and every vertex and edge of $P$ is contained in $Z_j$. Let $K\in \fset_j$ be the core that serves as the root of $T$. From the same arguments as before, the distance from $s(K)$ to $u$ in $Z_j^{K}$ is at most $R^c_{j}+1$, and the distance from $s(K)$ to $v$ in $Z_j^{K}$ is at most $R^c_{j}+1+2D\leq R^d_{j}+1$. Therefore, $u$ must lie in $T$.     
\end{proof}
        
        

        \paragraph{Responding to $\distquery_D(u,v)$.}  
        Recall that in a $\distquery_D(u,v)$, we are given two vertices $u$ and $v$ that lie in the same connected component of $G$. The algorithm needs to return either ``Yes'' or ''No'', such that, if ``Yes'' is returned then $\dist_G(u,v)\leq 2^{k+1}D+\log^{O(k)}n$ holds, and if ``No'' is returned, then $\dist_G(u,v)>2D$ holds.
        
        The algorithm for responding to this query is very similar to the one for $\pathquery_D(u,v)$, except that now we do not need to return the path itself. We check, in time $O(1)$, whether $H(u)$ is empty. If so, then we return ``yes'': since $u$ and $v$ are guaranteed to lie in the same connected component of $G$, and $u$ lies in a small and lonely connected component of $G$ (as it is not covered), from Observation~\ref{obs: small dont need centers}, $\dist_G(u,v)<D$ must hold. Assume now that $H(u)$ is non-empty. We inspect a tree $T$ of smallest rank in $H(u)$, and check, in time $O(1)$, whether $v\in V(T)$, by inspecting an appropriate entry from one of the arrays $A^1_v,\ldots,A^{r'}_v,A^L_v$, the choice of the array depending on the rank of $T$. If $v$ lies in $T$, then we return ``Yes''; from the above discussion, $\dist_G(u,v)\leq 2^{k+1}D+\log^{O(k)}n$ must hold. Otherwise, we return ``No''. From the analysis of $\pathquery_D$, if $\dist_G(u,v)\leq 2D$ and $u$ is covered by some tree $T$, then $v$ must also lie in the same tree. Therefore, if the algorithm returns ``No'', then we are guaranteed that $\dist_G(u,v)>2D$. The running time of the algorithm is $O(1)$.
        


==> SSSP_intro.tex <==
\section{SSSP}\label{sec: SSSP}

In this section, we consider decremental Single-Source Shortest
Paths ($\SSSP$) in  undirected \emph{weighted}
graphs. The problem is defined similarly to decremental $\APSP$, except that now we are given a source vertex $s$, and $\distquery$ and $\pquery$ are restricted to pairs $(u,v)$ of vertices where $u=s$ and $v$ is an arbitrary vertex.

We now provide an overview of previous work on this problem (see \Cref{tab:SSSP}  in Appendix \ref{sec: tables} 
for a summary). All algorithms below work in undirected graphs and have
$O(1)$ query time for $\dquery$. 


Even and Shiloach \cite{EvenS}
gave the first non-trivial  algorithm for decremental $\SSSP$ on unweighted
graphs. Their algorithm is \emph{exact}, deterministic (and hence adaptive-update),
and has $O(mn)$ total update time, which is also conditionally optimal.\footnote{Assuming the BMM conjecture~\cite{RodittyZ11}, or the OMV
conjecture~\cite{HenzingerKNS15}, there is no exact algorithm for \SSSP
with $O(mn^{1-\delta})$ total update time for any constant $\delta>0$.} Therefore, there is a line of work \cite{BernsteinR11,HenzingerKN14_soda,HenzingerKN14_focs} focusing on improving the running time by allowing $(1+\eps)$-approximation. 
In \cite{HenzingerKN14_focs}, Forster, Henzinger, and Nanongkai show a near-optimal $(1+\eps)$-approximation algorithm with $\Ohat(m\log L)$ total update time

in order to obtain faster algorithms we need to allow approximation.
The first algorithm for \SSSP to break the $O(mn)$ bound on total update time was by Bernstein
and Roditty \cite{BernsteinR11},  achieving a $(1+\epsilon)$-approximation in $O(n^{2+o(1)})$ total update time %
in unweighted graphs.
 This bound
was improved by Forster, Henzinger, and Nanongkai \cite{HenzingerKN14_soda}
to $O(n^{1.8+o(1)}+m^{1+o(1)})$. Shortly thereafter, the same authors
\cite{HenzingerKN14_focs} extended the algorithm to weighted graphs and improved
the running time to the essentially linear bound of $O(m^{1+o(1)}\log L)$, where
$L$ is the ratio of largest to smallest edge length. In all these algorithms, the query time for $\pquery$ is proportional to the number of edges in the returned path. Unfortunately, all of the above algorithms assume an oblivious adversary. 

It is an important open problem whether one can obtain total update time of $O(m^{1+o(1)}\log L)$ in the adaptive-update setting. If the answer to this question is positive, then, using known
reductions\footnote{Some of these reductions are only implicit in the literature. We make them explicit
in \Cref{sec:mincost} and \Cref{sec:more_app}.}, we immediately obtain near-linear time algorithms for a number of
flow and cut problems and algorithms for approximating treewidth. These reductions crucially require that the algorithm for decremental $\SSSP$
(1) works in weighted graphs; (2) handles adaptive updates;
and (3) support $\pquery$, that is, it can return an actual approximate
shortest path and not only the approximate distance.

The first adaptive-update algorithm to break the $O(mn)$ bound of Even-Shiloach on the total update time
 was shown by Bernstein and Chechik \cite{BernsteinChechik}.
Their algorithm is deterministic, with $\tilde{O}(n^{2})$ total
update time, though it can only handle unweighted graphs. They later showed another algorithm with total update time of
$\tilde{O}(n^{5/4}\sqrt{m})$ \cite{BernsteinChechikSparse}, which
is faster on sparse graphs. More recently, Bernstein \cite{Bernstein} extended the $\tilde{O}(n^{2})$-time algorithm to weighted graphs.
All these algorithms are deterministic, and therefore can handle adaptive updates. Unfortunately, they share
another drawback: they only support $\distquery$ but not $\pquery$.

Very recently, this issue was partially addressed by Chuzhoy and Khanna
\cite{fast-vertex-sparsest}, who extended the algorithm of \cite{Bernstein} by employing a new set of expander-based techniques. They obtain a randomized $(1+\epsilon)$-approximation
adaptive-update algorithm for weighted graphs, with  total expected update time $O(n^{2+O(1/\log\log n)}\cdot \frac{\log^{2}(1/\eps)\cdot\log L}{\eps^{2}})$ and expected query time $\tilde{O}(n\log L)$
for $\pquery$. As the algorithm can handle $\pquery$,
their results lead to new algorithms for approximate vertex-capacitated
maximum $s$-$t$ flow, minimum $s$-$t$ cut, and sparsest cut, which are the fastest currently known algorithms in
dense enough graphs.

There is still, however, one caveat. The algorithm in \cite{fast-vertex-sparsest}
only works in the \emph{vertex-decremental} setting,
where the underlying graph undergoes a sequence of vertex deletions
instead of edge deletions (when a vertex $v$ is deleted, all edges
incident to $v$ are deleted in one update operation). Observe that this variant
is a special case of the standard (edge)-decremental setting. Moreover,
vertex-decremental setting limits applications of the algorithm to flow/cut problems
to only the vertex-capacitated variants.

In this work, we improve the algorithm in \cite{fast-vertex-sparsest}
in two ways. We extend the algorithm to the edge-decremental setting, and improve its total expected update time by replacing a $n^{O(1/\log\log n)}$ factor by a $\poly\log n$ factor:\footnote{Since the algorithm of~\cite{Bernstein} supports $\distquery$, we only focus on supporting $\pquery$.}

\begin{theorem}
\label{thm: main for SSSP old}There is a randomized algorithm for \SSSP, that,
given a parameter $0<\epsilon<1$, and a simple undirected $n$-vertex
graph $G$ with lengths $\ell(e)>0$ on edges $e\in E(G)$, together
with a special source vertex $s\in V(G)$, such that $G$ undergoes
edge deletions, supports queries $\pquery(v)$ with
$(1+\eps)$-approximation factor. %

{} The algorithm works against an \textbf{adaptive}
adversary. The total expected running time of the algorithm is $O\left(n^{2}\cdot \frac{\poly\log n\cdot\log^{2}(1/\eps)\cdot\log L}{\eps^{2}}\right)$,
where $L$ is the ratio of largest to smallest edge length $\ell(e)$,
and each query is answered in expected time $O(n\cdot\poly\log n\cdot\log L\cdot\log(1/\eps))$.
\end{theorem}

To illustrate the power of \Cref{thm: main for SSSP}, we list some of its
applications to static graph problems:
\begin{corollary}
[Informal]\label{cor:application}There are randomized algorithms that obtain the following results in an $n$-vertex graph $G$: 
\begin{enumerate}
\item an $O(\log^{3}n)$-approximation for treewidth;
\item an $O(\log^{2}n)$-approximation for the most-balanced sparsest vertex cut; 
\item a $(1+\eps)$-approximation for maximum $s$-$t$ flow and its bounded-cost extension (this also implies a $(1+\eps)$-factor pseudo-approximation for min-cost $s$-$t$ flow; see Section~\ref{sec:mincost} for more details);
\item a $(1+\eps)$-approximation for maximum $k$-commodity flow and its bounded-cost
extension;
\item a $(1+\eps)$-approximation for concurrent $k$-commodity flow and its bounded-cost
extension; and
\item an $O(\frac{\log n}{\log\log n})$-approximation for congestion minimization
with $k$ demand pairs.
\end{enumerate}
The algorithms for (3)-(6) work in both the vertex-capacitated setting with arbitrary vertex capacities, and
the edge-capacitated setting with unit edge capacities.
The running time for the first three problems is ${\Ohat}(n^{2})$, and the running time for the last three problems is  ${\Ohat}(kn^{2})$.\footnote{
For simplicity, we hide $\poly(\log(BC)/\eps)$ factors, where $B$ is the ratio of largest to smallest cost on edges or vertices
and $C$ is the ratio of largest to smallest capacity on vertices; see \Cref{thm:mincost edge,thm:mincost vertex,cor:k concurrent flow,cor:k max flow,cor:congestion,cor:sparse cut,cor:treewidth} for the formal statements.}
\end{corollary}

All these applications follow from known (implicit) reductions \cite{RaghavanT87,BodlaenderGHK95,KRV}
or known techniques based on the multiplicative weight update framework
\cite{GK98,Fleischer00,fast-vertex-sparsest}. For many reductions
used in the proof of \Cref{cor:application}, we can plug in the previous vertex-decremental
algorithm of~\cite{fast-vertex-sparsest} as well, except that we would not obtain
(3)-(6) in the edge-capacitated setting, and we would obtain a slightly slower running time: either $O(n^{2+o(1)})$ and $O(kn^{2+o(1)})$. %
We now provide a brief comparison of these applications
with other known results. 

For treewidth, given a graph with $n$ nodes and treewidth $k$, previously known
algorithms either have running time that depends exponentially on $k$
\cite{flat-wall-RS,Amir01,Amir10,Bodlaender96,BodlaenderDDFLP16},
or have large polynomial running time \cite{BodlaenderGHK95,Amir01,Amir10,FeigeHL05}, providing a polylogarithmic approximation.
One exception is the algorithm by Fomin et al. \cite{FominLSPW18}, that
 computes an $O(k)$-approximation for treewidth in time $O(k^{7}n\log n)$.
Our algorithm is faster than that of \cite{FominLSPW18} when $k=\omega(n^{1/7+o(1)})$\footnote{
 Fast algorithms for the regime when the treewidth $k\leq n^{\eps}$ for a small constant $\eps$ have been recently developed for many 
 fundamental problems, including maximum matching, max flow, determinant, and linear system solvers.
 These algorithms are called \emph{fully-polynomial fixed parameter tractable} algorithms (see \cite{FominLSPW18,IwataOO18}).
 Most, if not all, of these algorithms rely on fast algorithms for approximating the treewidth when $k$ is a small polynomial in $n$.
}
and also gives a better approximation; see \Cref{tab:treewidth} in Appendix~\ref{sec: tables} for additional
details. For other flow-related problems, our algorithms are the fastest
when $m=\omega(n^{1.5+o(1)})$ and $k=O((m/n)^{2})$ in all problems,
except for the approximate maximum $s$-$t$ flow and $k$-commodity concurrent flow in the edge-capacitated setting; see \Cref{tab:edge flow}
and \Cref{tab:vertex flow}  in Appendix~\ref{sec: tables}  for detailed comparison.


==> header.tex <==

\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amstext}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{ntheorem}
\usepackage{graphicx}
\usepackage{url}
\usepackage{graphics}
\usepackage{colordvi}
\usepackage{subfigure}
\usepackage{xcolor}
\usepackage{comment}

\usepackage{array}
\usepackage{verbatim}
\usepackage{float}
\usepackage{multirow}

\RequirePackage[normalem]{ulem} %
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %
\providecommand{\DIFaddbegin}{} %
\providecommand{\DIFaddend}{} %
\providecommand{\DIFdelbegin}{} %
\providecommand{\DIFdelend}{} %
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %
\providecommand{\DIFaddbeginFL}{} %
\providecommand{\DIFaddendFL}{} %
\providecommand{\DIFdelbeginFL}{} %
\providecommand{\DIFdelendFL}{} %



\definecolor{ForestGreen}{rgb}{0.1333,0.5451,0.1333}
\definecolor{DarkRed}{rgb}{0.8,0,0}
\definecolor{Red}{rgb}{1,0,0}
\usepackage[linktocpage=true,
pagebackref=true,colorlinks,
linkcolor=DarkRed,citecolor=ForestGreen,
bookmarks,bookmarksopen,bookmarksnumbered]
{hyperref}

\usepackage{cleveref}



\textheight 9.3in \advance \topmargin by -1.0in \textwidth 6.7in
\advance \oddsidemargin by -0.8in
\newcommand{\myparskip}{3pt}
\parskip \myparskip









\newcommand{\SSSP}{\mbox{\sf{SSSP}}\xspace}
\newcommand{\APSP}{\mbox{\sf{APSP}}\xspace}
\newcommand{\MBCF}{\mbox{\sf{MBCF}}\xspace}

\newcommand{\connect}{\leadsto}
\newcommand{\highlightf}[2][red]{\fbox{\ensuremath{\textcolor{#1}{\mathbf #2}}}}

\newcommand{\MP}{\mbox{\sf Minimum Planarization}\xspace}
\newcommand{\MCN}{\mbox{\sf Minimum Crossing Number}\xspace}

\newcommand{\MS}{{\sf Machine Scheduling}\xspace}
\newcommand{\RMS}{{\sf Restricted Machine Scheduling}\xspace}
\newcommand{\CM}{{\sf Congestion Minimization}\xspace}
\newcommand{\ST}{{\sf Steiner Tree}\xspace}
\newcommand{\CD}{{\sf Cost-Distance}\xspace}
\newcommand{\PST}{{\sf Priority Steiner Tree}\xspace}
\newcommand{\FCNF}{{\sf FCNF}\xspace}
\newcommand{\AC}{{\sf Asymmetric $k$-Center}\xspace}
\newcommand{\kC}{{\sf $k$-Center}\xspace}
\newcommand{\dH}{{\sf $d$-Hypergraph-Cover}\xspace}
\newcommand{\kH}{{\sf $k$-Hypergraph-Cover}\xspace}
\newcommand{\GS}{{\sf Group-Steiner-Tree}\xspace}
\newcommand{\SC}{{\sf Set-Cover}\xspace}
\newcommand{\GAPSAT}{{\sf Gap-3SAT(5)}\xspace}
\newcommand{\clique}{{\sf Max-Clique}\xspace}
\newcommand{\ML}{{\sf Metric Labeling}\xspace}
\newcommand{\ZE}{{\sf 0-extension}\xspace}
\newcommand{\ZIE}{{\sf $(0,\infty)$-extension}\xspace}
\newcommand{\sat}{{\sf SAT}\xspace}
\newcommand{\mdc}{{\sf MDC}\xspace}
\newcommand{\csp}{{\sf HA-CSP}\xspace}

\newcommand{\Gr}[1]{G^{(#1)}}
\newcommand{\Hr}[1]{H^{(#1)}}

\newcommand{\pln}{\ensuremath{\poly\log n}}

\newcommand{\corepath}{\mbox{\sf{core-path}}}
\newcommand{\pquery}{\mbox{\sf{path-query}}\xspace}
\newcommand{\dquery}{\mbox{\sf{dist-query}}\xspace}
\newcommand{\pathquery}{\mbox{\sf{path-query}}\xspace}
\newcommand{\distquery}{\mbox{\sf{dist-query}}\xspace}
\newcommand{\VS}{\mbox{\sf{Vertex-Split}}}
\newcommand{\DE}{\mbox{\sf{Delete-Edge}}}
\newcommand{\CONN}{\mbox{\sf{CONN}}}
\newcommand{\CONNSF}{\mbox{\sf{CONN-SF}}}
\renewcommand{\path}{\mbox{\sf{path}}}
\newcommand{\EST}{\mbox{\sf{ES-Tree}}\xspace}
\newcommand{\ESTdel}{\mbox{\sf{EST-del}}\xspace}
\newcommand{\ESTs}{\mbox{\sf{ES-Trees}}\xspace}
\newcommand{\CONNIN}{\mbox{\sf{CONN-Insert}}}
\newcommand{\CONNDEL}{\mbox{\sf{CONN-Delete}}}
\newcommand{\conn}{\mbox{\sf{conn}}}

\newcommand{\splitsupernode}{\mbox{\sf{Split-Supernode}}}
\newcommand{\insertedges}{\mbox{\sf{Insert-Edges}}}
\newcommand{\opencenter}{\mbox{\sf{Open-Center}}}
        \newcommand{\movecenter}{\mbox{\sf{Move-Center}}}
\newcommand{\deledgecore}{\mbox{\sf{Delete-Edge-Core}}}
\newcommand{\deledgelayer}{\mbox{\sf{Delete-Edge-Layer}}}
\newcommand{\shortkpath}{\mbox{\sf{Short-Core-Path}}}
\newcommand{\shortpath}{\mbox{\sf{Short-Path}}}
\newcommand{\tocore}{\mbox{\sf{To-Core-Path}}}
\newcommand{\DSP}{\mbox{\sf{Proc-Degree-Pruning}}\xspace}
\newcommand{\algPS}{\mbox{\sf{Alg-Maintain-Pruned-Set}}\xspace}
\newcommand{\PDS}{\mbox{\sf{Proc-Degree-Pruning}}\xspace}
\newcommand{\DP}{\mbox{\sf{Proc-Degree-Pruning}}\xspace}
\newcommand{\hgl}{\ensuremath{\hat G^L}}
\newcommand{\CCD}{\mbox{\sf{Compute-Core-Decomp}}\xspace}
\newcommand{\OK}{\overline{K}}
\newcommand{\psii}{\psi_{s_i}}
\newcommand{\Psii}{\Psi_{s_i}}
\newcommand{\deledge}{\mbox{\sf{Delete-Edge}}\xspace}
\newcommand{\gapdegree}{12\xspace}
\newcommand{\gapU}{4\xspace}


\newcommand{\PSP}{\mbox{\sf{Proc-Path-Simplify}}\xspace}
\newcommand{\PCL}{\mbox{\sf{Proc-Construct-Layers}}\xspace}
\newcommand{\PLC}{\mbox{\sf{Proc-Construct-Layers}}\xspace}
\newcommand{\PDV}{\mbox{\sf{Proc-Delete-Vertex}}\xspace}
\newcommand{\FP}{\mbox{\sf{Proc-Find-Path}}\xspace}
\newcommand{\Lamda}{\Lambda}


\newcommand{\optmp}[1]{\mathsf{OPT}_{\mathsf{MP}}(#1)}
\newcommand{\optcro}[1]{\mathsf{OPT}_{\mathsf{cr}}(#1)}
\newcommand{\optcost}{\mathsf{OPT}_{\mathsf{cost}}}

\newcommand{\optcrosq}[1]{\mathsf{OPT}^{2}_{\mathsf{cr}}(#1)}
\newcommand{\algsc}{\ensuremath{{\mathcal{A}}_{\mbox{\textup{\footnotesize{ALN}}}}}\xspace}
\newcommand{\alphasc}{\ensuremath{\alpha_{\mbox{\textup{\footnotesize{ALN}}}}}}

\newcommand{\bad}{\mathsf{bad}}
\newcommand{\G}{{\mathbf{G}}}
\renewcommand{\H}{{\mathbf{H}}}
\newcommand{\bphi}{{\boldsymbol{\varphi}}}
\newcommand{\bpsi}{{\boldsymbol{\psi}}}
\newcommand{\RP}{{\sc 1R2P}\xspace}
\newcommand{\RV}{{\sc Raz Verifier}\xspace}

\newcommand{\size}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}}
\newcommand{\Dexp}[1]{\dexp\{#1\}}
\newcommand{\Tower}[2]{\operatorname{tower}^{(#1)}\{#2\}}
\newcommand{\logi}[2]{\operatorname{log}^{(#1)}{#2}}
\newcommand{\norm}[1]{\lVert #1\rVert}
\newcommand{\abs}[1]{\lvert #1\rvert}
\newcommand{\paren}[1]{\left ( #1 \right ) }
\newcommand{\union}{\cup}
\newcommand{\band}{\wedge}
\newcommand{\bor}{\vee}
\newcommand{\indeg}{\mathrm{in}\text{-}\mathrm{deg}}
\newcommand{\outdeg}{\mathrm{out}\text{-}\mathrm{deg}}
\newcommand{\invol}{\mathrm{in}\text{-}\mathrm{vol}}
\newcommand{\outvol}{\mathrm{out}\text{-}\mathrm{vol}}
\newcommand{\vol}{\mathrm{vol}}

\newcommand{\psd}{\succeq}


\newcommand{\rank}{\operatorname{rank}}
\newcommand{\event}{{\cal{E}}}

\newcommand{\wrt}{with respect to }

\renewcommand{\P}{\mathcal{P}}
\newcommand{\NP}{\mbox{\sf NP}}
\newcommand{\PCP}{\mbox{\sf PCP}}
\newcommand{\ZPP}{\mbox{\sf ZPP}}
\newcommand{\polylog}[1]{\mathrm{polylog(#1)}}
\newcommand{\DTIME}{\mbox{\sf DTIME}}

\newcommand{\opt}{\mathsf{OPT}}


\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\sse}{\subseteq}

\newcommand{\B}{{\mathcal{B}}}
\newcommand{\tset}{{\mathcal T}}
\newcommand{\iset}{{\mathcal{I}}}
\newcommand{\pset}{{\mathcal{P}}}
\newcommand{\qset}{{\mathcal{Q}}}
\newcommand{\lset}{{\mathcal{L}}}
\newcommand{\bset}{{\mathcal{B}}}
\newcommand{\aset}{{\mathcal{A}}}
\newcommand{\cset}{{\mathcal{C}}}
\newcommand{\fset}{{\mathcal{F}}}
\newcommand{\dset}{{\mathcal{D}}}
\newcommand{\mset}{{\mathcal M}}
\newcommand{\jset}{{\mathcal{J}}}
\newcommand{\xset}{{\mathcal{X}}}
\newcommand{\wset}{{\mathcal{W}}}

\newcommand{\yset}{{\mathcal{Y}}}
\newcommand{\rset}{{\mathcal{R}}}

\newcommand{\I}{{\mathcal I}}
\newcommand{\hset}{{\mathcal{H}}}
\newcommand{\sset}{{\mathcal{S}}}
\newcommand{\kset}{{\mathcal{K}}}
\newcommand{\zset}{{\mathcal{Z}}}
\newcommand{\notu}{\overline U}
\newcommand{\nots}{\overline S}

\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{rem}[theorem]{Remark}
\newtheorem{assumption}{Assumption}[section]
\newtheorem*{definition}{Definition.}
\newtheorem*{defn}{Definition.}
\newenvironment{proof}{\par {\bf Proof:}}{\hfill\stopproof}
\def\stopproof{\square}
\def\square{\vbox{\hrule height.2pt\hbox{\vrule width.2pt height5pt \kern5pt
\vrule width.2pt} \hrule height.2pt}}

\newenvironment{proofof}[1]{\noindent{\bf Proof of #1.}}%
        {\hfill\stopproof}

\providecommand{\tabularnewline}{\\}
\floatstyle{ruled}
\newfloat{algorithm}{tbp}{loa}
\providecommand{\algorithmname}{Algorithm}
\floatname{algorithm}{\protect\algorithmname}

\newcommand{\scale}[2]{\scalebox{#1}{#2}}

\newcommand{\fig}[1]{
\begin{figure}[h]
\rotatebox{0}{\includegraphics{#1}}
\end{figure}}

\newcommand{\figcap}[2]
{
\begin{figure}[h]
\rotatebox{270}{\includegraphics{#1}} \caption{#2}
\end{figure}
}

\newcommand{\scalefig}[2]{
\begin{figure}[h]
\scalebox{#1}{\includegraphics{#2}}
\end{figure}}

\newcommand{\scalefigcap}[3]{
\begin{figure}[h]
\scalebox{#1}{\rotatebox{0}{\includegraphics{#2}}} \caption{#3}
\end{figure}}

\newcommand{\scalefigcaplabel}[4]{
\begin{figure}[h]
 \scalebox{#1}{\includegraphics{#2}}\caption{#3\label{#4}}
\end{figure}}




\fboxsep=16pt
\newenvironment{prog}[1]{
        \begin{minipage}{5.8 in}
                \begin{center}
                        {\sc #1}
                \end{center}
        }
        {
\end{minipage}}

\newcommand{\program}[2]{\fbox{\vspace{2mm}\begin{prog}{#1} #2 \end{prog}\vspace{2mm}}}



\renewcommand{\phi}{\varphi}
\newcommand{\eps}{\epsilon}
\newcommand{\Sum}{\displaystyle\sum}
\newcommand{\half}{\ensuremath{\frac{1}{2}}}

\newcommand{\poly}{\operatorname{poly}}
\newcommand{\dist}{\mbox{\sf dist}}
\global\long\def\apxdist{\widetilde{\mathsf{dist}}}
\global\long\def\inc{\mathtt{inc}}
\global\long\def\edge{\mathtt{Edges}}
\global\long\def\edges{\mathtt{Edges}}
\newcommand{\reals}{{\mathbb R}}

\newcommand{\rn}{\reals^n}
\newcommand{\rk}{\reals^k}
\newcommand{\newsigma}{\Sigma^{d^{\ceil{t/2}}}}
\newcommand{\R}{\ensuremath{\mathbb R}}
\newcommand{\Z}{\ensuremath{\mathbb Z}}
\newcommand{\N}{\ensuremath{\mathbb N}}
\newcommand{\F}{\ensuremath{\mathbb F}}
\newcommand{\fm}{\enshuremath{\mathbb F}^m}
\newcommand{\func}{:{\mathbb F}^m\rightarrow {\mathbb F}}

\newcommand{\T}{\ensuremath{\mathcal T}}
\newcommand{\A}{\ensuremath{\mathcal A}}

\newcommand{\one}{{\mathbf{1}}}


\newcommand{\expect}[2][]{\text{\bf E}_{#1}\left [#2\right]}
\newcommand{\prob}[2][]{\text{\bf Pr}_{#1}\left [#2\right]}

\newcommand{\four}[1]{\widehat {#1}}
\newcommand{\fourf}{\widehat {f}}
\newcommand{\fourg}{\widehat {g}}
\newcommand{\chisx}{\chi_S(x)}
\newcommand{\chitx}{\chi_T(x)}
\newcommand{\chisy}{\chi_S(y)}
\newcommand{\chity}{\chi_T(y)}
\newcommand{\chiwx}{\chi_W(x)}
\newcommand{\chiwy}{\chi_W(y)}
\newcommand{\chis}{\chi_S}
\newcommand{\chit}{\chi_T}
\newcommand{\chiw}{\chi_W}
\newcommand{\chisminust}{\chi_{S\triangle T}}

\newenvironment{properties}[2][0]
{\renewcommand{\theenumi}{#2\arabic{enumi}}
\begin{enumerate} \setcounter{enumi}{#1}}{\end{enumerate}\renewcommand{\theenumi}{\arabic{enumi}}}


\setlength{\parskip}{2mm} \setlength{\parindent}{0mm}


\newcommand{\fillin}{\textcolor{red}{\sc \bf{[Fill in]}}}
\renewcommand{\check}{\textcolor{red}{\sc \bf{[Check!]}}}
\newcommand{\explain}{\textcolor{red}{\sc \bf{[Explain]}}}


\newcommand{\notsat}[1]{\overline{\text{SAT}(#1)}}
\newcommand{\notsats}[2]{\overline{\text{SAT}_{#1}(#2)}}

\newcommand{\sndp}{\mbox{\sf SNDP}}
\newcommand{\ecsndp}{\mbox{\sf EC-SNDP}}
\newcommand{\vcsndp}{\mbox{\sf VC-SNDP}}
\newcommand{\kec}{k\mbox{\sf -edge connectivity}}
\newcommand{\kvc}{k\mbox{\sf -vertex connectivity}}
\newcommand{\sskec}{\mbox{\sf single-source}~k\mbox{\sf -edge connectivity}}
\newcommand{\sskvc}{\mbox{\sf single-source}~k\mbox{\sf -vertex connectivity}}
\newcommand{\subkvc}{\mbox{\sf subset}~k\mbox{\sf -vertex connectivity}}
\newcommand{\oneec}{1\mbox{\sf -edge connectivity}}
\newcommand{\onevc}{1\mbox{\sf -vertex connectivity}}
\newcommand{\kvcssp}{k\mbox{\sf -vertex-connected spanning subgraph problem}}


\newcommand{\dmax}{d_{\mbox{\textup{\footnotesize{max}}}}}
\newcommand{\LCD}{{\sf{LCD}}\xspace}
\newcommand{\lcd}{{\sf{LCD}}\xspace}
\newcommand{\td}{\widetilde{\deg}}
\newcommand{\tlambda}{\tilde \Lambda}
\newcommand{\out}{\operatorname{out}}
\newcommand{\cro}{\operatorname{cr}}
\newcommand{\cre}{\operatorname{cre}}
\global\long\def\mincost{\mathtt{mincost}}
\global\long\def\Ohat{\widehat{O}}
\global\long\def\Otil{\tilde{O}}
\global\long\def\Omegahat{\widehat{\Omega}}
\global\long\def\Ball{\mathrm{Ball}}
\global\long\def\cutorcert{\textsc{CutOrCertity}}
\global\long\def\termMatching{\textsc{TerminalMatching}}
















\def\thatchapholnew#1{#1}

\def\thatchaphol#1{\marginpar{$\leftarrow$\fbox{T}}\footnote{$\Rightarrow$~{\sf #1 --Thatchaphol}}}
\newcommand{\mynote}[1]{\textcolor{red}{\sc\bf{[#1]}}}

\newcommand{\mmynote}[1]{\textcolor{red}{\sc\bf{[#1]}}}


\global\long\def\ex{\mathrm{ex}}
\global\long\def\ab{\mathrm{ab}}
\global\long\def\ball{\mathrm{Ball}}
\global\long\def\val{\mathrm{val}}
